Fast Algorithms for the Maximum Clique Problem on Massive Graphs with Applications to Overlapping Community Detection

The maximum clique problem is a well known NP-Hard problem with applications in data mining, network analysis, information retrieval and many other areas related to the World Wide Web. There exist several algorithms for the problem with acceptable runtimes for certain classes of graphs, but many of them are infeasible for massive graphs. We present a new exact algorithm that employs novel pruning techniques and is able to find maximum cliques in very large, sparse graphs quickly. Extensive experiments on different kinds of synthetic and real-world graphs show that our new algorithm can be orders of magnitude faster than existing algorithms. We also present a heuristic that runs orders of magnitude faster than the exact algorithm while providing optimal or near-optimal solutions. We illustrate a simple application of the algorithms in developing methods for detection of overlapping communities in networks.

==> arXiv Submission/abs.tex <==
%%% AHG: testing git pull
The maximum clique problem is a well known NP-Hard problem with
applications in data mining, network analysis, information retrieval and many other
areas related to the World Wide Web.
There exist several algorithms for the problem with acceptable runtimes for
certain classes of graphs, but many of them are infeasible for massive graphs. 
We present a new exact algorithm that employs novel pruning techniques and 
is able to find maximum cliques in very large, sparse graphs quickly. 
Extensive experiments on different kinds of synthetic and 
real-world graphs show that our new algorithm can be orders of magnitude 
faster than existing algorithms.
We also present a heuristic that runs orders of magnitude faster than 
the exact algorithm while providing optimal or near-optimal solutions.
We illustrate a simple application of the algorithms in developing methods for
detection of overlapping communities in networks.



==> arXiv Submission/algorithms.tex <==
\section{The New Algorithms}
\label{sec:algorithms}
%\vspace{-6pt}
We describe in this section new algorithms that overcome the shortcomings mentioned earlier; 
the new algorithms use additional pruning strategies, maintain simplicity, and 
avoid a sequential computational order.
We begin by first introducing the following notations.
%Let $G = (V,E)$ denote a simple undirected graph, and let $n = \left|V\right|$ and $m = \left|E\right|$. 
We identify the $n$ vertices of the input graph $G=(V,E)$ as $\{v_1, v_2, \ldots, v_n\}$.  
The set of vertices adjacent to a vertex $v_i$, the set of its neighbors, is denoted by $N(v_i)$.
And the degree of the vertex $v_i$, the cardinality of $N(v_i)$, is 
denoted by $d(v_i)$. In our algorithm, the degree is computed once for each vertex at the beginning.

%\vspace{-10pt}
\subsection{The Exact Algorithm}
\label{subsec:exact}
%\vspace{-4pt}

Recall that the maximum clique in a graph can be found by computing the largest clique containing each vertex and picking the largest among these. 
A key element of our exact algorithm is that during the search for the largest clique containing a given vertex, vertices that cannot form cliques larger than the current maximum 
clique are {\em pruned}, in a hierarchical fashion. 
The method is outlined in detail in Algorithm \ref{alg:mClq}. 
Throughout, the variable $max$ stores the size of the maximum clique found 
thus far. Initially it is set to be equal to the lower bound $lb$ provided as an input parameter.
It gives the maximum clique size when the algorithm terminates.

\begin{figure}
%\vspace{14pt}
\hrule
\vspace{6pt}
\begin{spacing}{\algospacing}
{
{\small
\captionof{algorithm}{{\protect\small Algorithm for finding the maximum clique of a given graph.
{\it Input}: Graph $G = \left (V, E\right )$, lower bound on clique $lb$ (default, 0). {\it Output}: Size of maximum clique.}}\label{alg:mClq}
\vspace{-5pt}
\hrule
\vspace{6pt}

\noindent\begin{minipage}{.5\textwidth}
\vspace{-12pt}
\begin{algorithmic}[1]
\Procedure {MaxClique}{$G=\left (V,E\right )$, $lb$}
\State $max \leftarrow lb$
\For{$i:1$ to $n$}
%\If{$degree(v_i) < maxClq$} 
%\State continue \Comment{{\small Pruning 1}}
%\EndIf
\If{$d(v_i) \ge max$} \Comment{{\footnotesize Pruning 1}} \label{pr1}
\State $U \leftarrow \emptyset$
\For{each $v_j \in N(v_i)$}
\If{$j > i$} \Comment{{\footnotesize Pruning 2}} \label{prOld}
\If{$d(v_j) \ge max$} \Comment{{\footnotesize Pruning 3}} \label{pr2}
\State $U \leftarrow U \cup \{v_j\}$ 
\EndIf
\EndIf
\EndFor

\State \textsc{Clique}$(G, U, 1)$ \label{subCall}
\EndIf

\EndFor
\EndProcedure
\end{algorithmic}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\captionof*{algorithm}{{\em Subroutine}}
\vspace{-6pt}
\begin{algorithmic}[1]
\Procedure {Clique}{$G=\left (V,E\right )$, $U$, $size$}

\If{$U = \emptyset$}
\If{$size > max$} 
\State $max \leftarrow size$ \label{critical}
\EndIf
\State {\bf return}
\EndIf

\While{$\left|U\right| > 0$}
\If{$size + \left|{U}\right| \le max$} \Comment{{\footnotesize Pruning 4}} \label{pr3}
\State {\bf return} 
\EndIf

\State Select any vertex $u$ from $U$ 
%of maximum degree in $G$

\State $U \leftarrow U \setminus \{u\} $
\State $N'(u):= \{w | w \in N(u) \wedge d(w) \ge max\}$  \Comment{{\footnotesize Pruning 5}} \label{pr4}
\State \textsc{Clique}$( G, U \cap N'(u), size + 1)$
\EndWhile

\EndProcedure
\end{algorithmic}
\end{minipage}
}
}
\end{spacing}
\vspace{8pt}
\hrule
%\vspace{10pt}
\end{figure}

To obtain the largest clique containing a vertex $v_i$, 
it is sufficient to consider only the neighbors of $v_i$. 
The main routine {\sc MaxClique} thus generates  for each 
vertex $v_i \in V$ a set $U \subseteq N(v_i)$ 
(neighbors of $v_i$ that survive pruning) and calls the subroutine \clq\ on $U$.  
The subroutine \clq\ goes through every relevant clique containing $v_i$ 
in a recursive fashion and returns the largest.
%, and a more elaborate explanation can be found there. 
We use $size$ to maintain the size of the clique found at any point through the recursion.
Since we start with a clique of just one vertex, the value of $size$ is set to one initially, 
when \clq\ is called (Line \ref{subCall}, {\sc MaxClique}).


Our algorithm consists of several pruning steps.
Pruning 1 (Line \ref{pr1}, {\sc MaxClique}) 
filters vertices having strictly fewer neighbors than the size of the maximum clique already computed. These vertices can be ignored, since even if a clique were to be found, its size would not be larger than $max$.
%at most one greater than its degree, which would still be less than $max$. 
While forming the neighbor list $U$ for a vertex $v_i$, we include only those of $v_i$'s 
neighbors for which the largest clique containing them has not been found 
(Pruning 2; Line \ref{prOld}, {\sc MaxClique}), 
to avoid recomputing previously found cliques.  
Pruning 3 (Line \ref{pr2}, {\sc MaxClique})
excludes vertices $v_j \in N(v_i)$  that have degree less than the current value of $max$, since any such vertex could not form a clique of size larger than $max$.
%This pruning step is valid because it is not possible to form a clique containing both $v_j$ and $v_i$ and still have size greater than $max$ as that would require each vertex of the clique to have degree greater than $max$, which is not the case for $v_j$. 
Pruning 4 (Line \ref{pr3}, {\sc Clique})
checks for the case where even if all vertices of $U$ were added to get a clique, its size would not exceed that of the largest clique encountered so far in the search, $max$. 
Pruning 5 (Line 11, {\sc Clique})
reduces the number of comparisons needed to generate the intersection set in Line 12.
Note that the routine \clq\ is similar to the 
Carraghan-Pardalos algorithm \cite{pardalos}; Pruning 5 accounts for the main difference.
Also, Pruning 4 is used in most existing algorithms, whereas Prunings 1, 2, 3 and 5 are not.

\subsection{The Heuristic}
\label{subsec:heuristic}

\begin{figure}
\vspace{10pt}
\hrule
\vspace{6pt}
\begin{spacing}{\algospacing}
{
{\small
\captionof{algorithm}{{\protect\small Heuristic for finding the maximum clique in a graph.
{\it Input}: Graph $G = \left (V, E\right )$. {\it Output}: Approximate size of maximum clique.}}\label{alg:mClqHeu}
\vspace{-5pt}
\hrule
\vspace{6pt}

\noindent\begin{minipage}{.5\textwidth}
\vspace{12pt}
\begin{algorithmic}[1]
\Procedure {MaxCliqueHeu}{$G=\left (V,E\right )$}
\For{$i:1$ to $n$}
%\If{$degree(v_i) < maxClq$} 
%\State continue \Comment{{\small Pruning 1}}
%\EndIf
\If{$d(v_i) \ge max$}
\State $U \leftarrow \emptyset$
\For{each $v_j \in N(v_i)$}
\If{$d(v_j) \ge max$} 
\State $U \leftarrow U \cup \{v_j\}$ 
\EndIf
\EndFor

\State \textsc{CliqueHeu}$(G, U, 1)$
\EndIf
%\EndIf

\EndFor
\EndProcedure
\end{algorithmic}
\end{minipage}%
\begin{minipage}{.5\textwidth}
\captionof*{algorithm}{{\em Subroutine}}
\vspace{-7pt}
\label{alg:clqHeu}
\begin{algorithmic}[1]
\Procedure {CliqueHeu}{$G=\left (V,E\right )$, $U$, $size$}

\If{$U = \emptyset$}
\If{$size > max$}
\State $max \leftarrow size$
\EndIf
\State {\bf return}
\EndIf

%\While{$U > \emptyset$}
%\If{$size + \left|{U}\right| <= max$} 
%\State \bf{return} \Comment{{\small Pruning 3}}
%\EndIf

%\State $i:=max\{j \mid v_j \in U\}$
\State Select a vertex $u \in U$ of maximum degree in $G$ \label{maxDsel}
%\State $U \leftarrow U \setminus u$
\State $U \leftarrow U \setminus \{u\} $
\State $N'(u):= \{w | w \in N(u) \wedge d(w) \ge max\}$  \label{pr4}
\State \textsc{CliqueHeu}$( G, U \cap N'(u), size + 1)$

%\State \textsc{CliqueHeu}$(G, U \cap N(u), size + 1)$
%\State return
%\EndWhile

\EndProcedure

\end{algorithmic}
\end{minipage}
}
}
\end{spacing}
\vspace{8pt}
\hrule
%\vspace{14pt}
\end{figure}



The exact algorithm examines all relevant cliques containing every vertex.
Our heuristic, shown in Algorithm \ref{alg:mClqHeu}, considers only {\em one} neighbor
with {\em maximum degree} at each step instead of recursively considering {\em all} neighbors 
from the set $U$, and thus is much faster. The vertex with maximum degree is chosen
for this intuitive reason: in a relatively fairly connected subgraph, a vertex with the maximum degree
is more likely to be a member of the largest clique containing that vertex
compared to any other.
%The subset considered is the one with high likelihood to contain the largest clique.  
 %The main routine is very similar to the main routine in Algorithm \ref{alg:mClq}. The subroutine \clqh\ considers only the {\em maximum degree} neighbor at each step instead of recursively considering all neighbors from the set $U$. Since we are looking for the largest clique containing each vertex, the maximum degree vertex is more likely to be a member of the largest clique compared to the other vertices. The effect of choosing the maximum degree vertex as opposed to any random vertex will be analyzed in Section~\ref{sec:exp-heuristic}.
%The pruning steps in Algorithm \ref{alg:mClqHeu}, are otherwise the same as in Algorithm \ref{alg:mClq}, unless not applicable (Pruning 2 and 4).
%We note that Turner \cite{Turner88} uses an algorithm similar in spirit to the subroutine of Algorithm \ref{alg:mClqHeu} in his coloring algorithm. 


%\vspace{-10pt}
\subsection{Complexity}
\label{subsec:complexity}
%\vspace{-4pt}

The exact algorithm, Algorithm \ref{alg:mClq}, examines for every vertex $v_i$ all candidate cliques containing the vertex $v_i$ in its search for the largest clique. Its time complexity is exponential in the worst case. The heuristic, Algorithm \ref{alg:mClqHeu}, loops over the $n$ vertices, each time possibly
calling the subroutine \clqh, which effectively is a loop that runs until the set $U$ is empty. 
Clearly, $|U|$ is bounded by the max degree $\Delta$ in the graph.  
%In the worst case, every vertex we consider might be connected to all other vertices in $G$, in which case $\left|U\right| = n-1$. 
The subroutine also includes the computation of a neighbor list, whose runtime is bounded by 
$O(\Delta)$.
% which in the worst case is $O(n)$. 
Thus, the time complexity of the heuristic is bounded by $O(n\cdot \Delta^{2})$.
%$O(n^3)$.
%\vspace{-8pt}

\subsection{Graph Data Structure}
\label{subsec:implementation}

Our implementation uses a simple adjacency list representation to store the graph. This is done by maintaining two arrays. Given a graph $G=(V,E)$, with its vertices numbered from $0$ to $|V|-1$, the edge array maintains the concatenated list of sorted neighbors of each vertex. The size of this array is $2|E|$. The vertex array is $|V|$ elements long, one for each vertex in sequential order, and each element points (stores the array index) to starting point of its neighbor list in the edge array. 
%In addition to the list of neighbors, the number of neighbors can also be easily obtained from our data structure. 
Figure \ref{fig-implementation} shows our representation and data structure used for a sample graph.

\begin{figure}
  \centering
    \includegraphics[scale=0.28]{implementation.eps}
\caption{The adjacency list data structure used in our implementation shown for a sample graph. Each element in the vertex array stores the index to the starting element of its neighbor list in the edge array.}
\label{fig-implementation}
\end{figure}



==> arXiv Submission/applications2.tex <==
\section{Clique Algorithms and Community Detection}
\label{sec:applications}

%In this section we demonstrate how clique finding algorithms can be used as parts of methods for detecting overlapping communities in networks. 
In this section we demonstrate how clique finding algorithms can be used for detecting overlapping communities in networks. 


{\bf Background. }
Most community detection algorithms are designed to identify mutually independent communities in a given network and therefore are not suitable for detecting overlapping communities. Yet, in many real-world networks, it is natural to find vertices (or members) that belong to more than one group (or community) at the same time.

Palla et al.~\cite{cite-key} introduced the Clique Percolation Method (CPM) 
as one effective approach for detecting overlapping communities in a network. 
The basic premise in CPM is that a typical community is likely to be made up of several cliques that share many of their vertices.  
We recall a few notions defined in \cite{cite-key} to make this more precise.
A clique of size $k$ is called a {\em $k$-clique}, and   
two $k$-cliques are called {\em adjacent} if they share $k - 1$ nodes. 
A {\em $k$-clique community} is a union of all $k$-cliques that can be reached 
from each other through a series of adjacent $k$-cliques. 
%Further, a {\em $k$-clique chain} is the union of a sequence of adjacent $k$-cliques, and two $k$-cliques are said to be $k$-clique-connected if they are parts of a $k$-clique chain. 
With these notions at hand, Palla et al. devise a method to extract such $k$-clique communities of a network. %which  are essentially the $k$-clique connected components of the network; 
Note that, by definition, $k$-clique communities allow for overlaps, i.e. common vertices can be shared by the  communities.
%Palla et al observe that the $k$-clique communities are equivalent to the $k$-clique connected components of the network; note that, by definition, $k$-clique communities allow for overlaps between communities to exist.

The CPM algorithm is illustrated in Figure \ref{fig-cpm}. Given a graph, we first extract all cliques of size $k$; for this example we choose $k$=3. This is followed by generating the {\it clique graph}, where each $k$-clique in the original graph is represented by a vertex. An edge is added between any two $k$-cliques in the clique graph that are adjacent. For the case $k$=3, this means an edge is added between any two 3-cliques in the clique graph that share two common vertices (of the original graph). The connected components in the clique graph represent a community, and the actual members of the community are obtained by gathering the vertices of the individual cliques that form the connected component. In our example in Figure \ref{fig-cpm}, we obtain two communities, which share a common vertex (vertex 2), forming an overlapping community structure.


\begin{figure}%[h!]
  \centering
    %\includegraphics[width=1\textwidth]{communities_fb.pdf}
    \includegraphics[scale=0.45]{cpm.eps}
    
%\vspace{-30pt}
  \caption{Illustration of overlapping community detection by the Clique Percolation Method (CPM) algorithm on a sample graph. Steps involved are 1) Detecting the $k$-cliques 2) Forming the clique-graph 3) Merging members of the connected components in the clique-graph to obtain the $k$-clique communities. In this example, node 2 is shared by the two communities formed, resulting in an overlapping structure.}
\label{fig-cpm}
\end{figure}
%\vspace{-10pt}



A large clique of size $q \geq k $ contains $\binom{q}{k}$ different {\em k-cliques}.
An algorithm that tries to locate the $k$-cliques individually and examine the adjacency
between them can therefore be very very slow for large networks. 
Palla et al. make two observations that help one come up with a better strategy.
First, a clique of size $q$ is clearly a $k$-clique connected subset for any $k \leq q$. 
Second, two large cliques that share at least $k-1$ nodes form one $k$-clique connected component as well.
Leveraging these, the strategy of Palla et al. avoids searching for $k$-cliques individually
and instead first locates the large cliques in the network and then looks for the $k$-clique connected subsets of given $k$ (that is, the $k$-clique communities) by studying the overlap between them.
More specifically, their algorithm first constructs a symmetric {\em clique-clique overlap matrix}, 
in which each row represents a large (to be precise a maximal) clique, 
each matrix entry is equal to the number of common nodes between the two corresponding cliques, and each diagonal entry is equal to the size of the clique. 
The $k$-clique communities for a given $k$ are then equivalent to connected 
clique components in which the neighboring cliques are linked to each other by at least $k-1$ common nodes. Palla et al. then find these components by erasing every off-diagonal entry smaller than $k-1$ and every diagonal entry smaller than $k$ in the matrix, replacing the remaining elements by one, and then carrying out a component analysis of this matrix. The resulting separate components are equivalent to the different $k$-clique communities.
       

%detects communities by merging overlapping sets of adjacent cliques. The first step in the algorithm is to identify all cliques of size $k$ in the given graph. This is typical done by detecting all maximal cliques in the graph. Then, a new graph is constructed such that each vertex represents one of these $k$-cliques. Two nodes in this new graph are considered to be connected if the $k$-cliques that represent them share $k$?1 members. The cliques of the connected components in the new graph are merged into communities. Since a vertex can occur in more than one $k$-cliques simultaneously, this results in an overlapping communities structure.

%\subsection{Our Method}

{\bf Our Method. } We devised an algorithm based on a similar idea as the procedure
above, but using a variant of our heuristic maximum clique-algorithm 
(Algorithm 2) for the core clique detection step. 

The standard CPM in essence presupposes finding {\em all} maximal cliques in a network.
The number of maximal cliques in a network can in general be exponential in the number of nodes $n$ in the network. In our method, we work instead with a smaller set of maximal cliques. In particular, the basic variant of our method considers exactly one clique per vertex, the largest of all the maximal cliques that it belongs to. Clearly, this can be too restrictive a requirement and may fail to add deserving members to a $k$-clique community. 
To allow for more refined solutions, we include a parameter $c$
in the method that tells us how many additional cliques per vertex would be considered.
The case $c=0$ corresponds to no additional cliques than the largest maximal clique containing the vertex. The case $c\geq1$ corresponds to $c$ additional maximal cliques (each of size at least $k$)
per vertex. Hence, in total, $n(c+1)$ cliques will be collected. For a particular vertex $v$, the largest maximal clique containing it 
can be heuristically obtained by exploring the neighbor of $v$ with {\em maximum degree} 
in the corresponding step in Algorithm 2.
In contrast, to obtain the other maximal cliques involving $v$ (case $c\geq1$),
we explore a {\em randomly} chosen neighbor of $v$, regardless of its degree value.



%The intuition for this follows from the fact that, in  CPM, many $k$-cliques which are $k$-clique-connected are merged into a single community. If we consider one such $k$-clique-community, it would naturally include the largest clique of size greater than or equal to $k$, that can be formed with a subset of its vertices. Hence, all large cliques of size greater than or equal to $k$ would certainly be contained within one of the $k$-clique-communities. 

%Hence, we extended our heuristic such that it returns the largest clique (not just the size) containing each node. However, only considering the largest cliques containing each vertex is clearly not enough, since there could be other vertices in a $k$-clique-community that does not belong to such large cliques, but could still be $k$-clique-connected to it. We need to consider additional maximal cliques in order to include these vertices. Hence, we introduced a parameter $c$, which essentially runs the heuristic $c$ additional times using a random choice of vertex at each step instead of picking the vertex with the largest degree. Assuming no duplicates, in total, $(c+1) \times n$ cliques would be collected, $n$ from the largest-degree-vertex selection iteration, and $c \times n$ from the random-vertex selection iterations. Since it is quite possible to produce duplicate cliques, the total number of cliques collected is typically lesser than $(c+1) \times n$.
%In addition, given a value of $k$, it is not necessary to look for cliques that are smaller than size $k$. We do this by replacing all occurrences of $max$ with $k-1$in Algorithm 2 which discards these. (We also remove Lines 2 and 3 as we now don't need to keep track of the maximum clique size.) Once the cliques are collected, we perform a standard component analysis of the clique-clique overlap matrix to obtain the communities.


%In order to make merging of cliques more ``aggressive'', we also included an option for extracting cliques other than the {\em largest}. 
%win the network since every smaller $k$-clique in it would also be $k$-clique-connected. 

%In order to make merging of cliques more ``aggressive'', we also included an option for extracting cliques other than the {\em largest}. 
%We implemented this by introducing a parameter $c$, which essentially runs the heuristic $c$ additional times using a random choice of vertex at each step instead of picking the vertex with the largest degree. 


%We also modified the pruning steps by discarding cliques that cannot be more than size $k$, instead of the maximum clique size. Since we only look for cliques that overlap at least by $k$ nodes, we can safely prune these out. This is achieved by replacing all occurrences of $max$ in Algorithm 2???, and removing Lines (2 and 3???) as we now don't need to keep track of the maximum clique size. 

%\subsection{Test on Synthetic Networks}

{\bf Test on Synthetic Networks. } We tested our algorithm on the LFR benchmarks\footnote{http://sites.google.com/site/andrealancichinetti/files} proposed in \cite{2008PhRvE..78d6110L}. These benchmarks have the attractive feature that they allow
for generation of synthetic networks with known communities (ground truth).
We generated graphs with $n$ = 1000 nodes, average degree $K$ = 10, and power law exponents $\tau_1$ = 2 and $\tau_2$ = 1 in the LFR model. We set the maximum degree $K_{max}$ to 50, and the minimum and maximum community sizes $C_{min}$ and $C_{max}$ to 20 and 50, respectively. We used two far-apart values each for the mixing parameter $\mu$, the fraction of overlapping nodes $O_n$, and the number of communities each overlapping node belongs to $O_m$. Specifically, for $\mu$ we used 0.1 and 0.3, for $O_n$ we used 10$\%$ and 50$\%$, and for $O_m$ we used 2 and 8. 
All together, these combinations of parameters resulted in eight graphs in the testbed.
%, which is of the same order as most large real-world social networks. 
%We chose to vary these as opposed to the others since these would have the most profound impact on the network topology for overlapping community detection. 
%These benchmarks introduce heterogeneity into degree and community size distributions of a network. These distributions are governed by power laws with exponents $\tau_1$ and $\tau_2$, respectively. It allows the generation of overlapping communities using the parameters, $O_n$, the fraction of overlapping nodes and $O_m$, the number of communities each overlapping node is assigned to. It also provides other parameters to control the network topology, such as the mixing parameter $\mu$, which is the expected fraction of links through which a node connects to other nodes in the same community, the average degree $K$, the maximum degree $K_{max}$, the maximum community size $C_{max}$, and the minimum community size $C_{min}$. 

%We evaluated the performance of our algorithm using the {\it Omega Index} \cite{doi:10.1207/s15327906mbr2302_6} which is the overlapping version of the Adjusted Rand Index (ARI) \cite{ARI_paper_1985}.
%which is a metric to compare how well two sets of clusters or communities agree with each other.
%, and it considers pairs of nodes belonging to the same number of clusters (possibly none) to compute the index.

%We define the set of clusters found as a cover $C=\{c_1, c_2, ..., c_k\}$ [Lancichinetti et al. 2009], where $k$ is the number of clusters found.In the case of overlapping communities, a node may belong more than one cluster. Let $N1$ and $N2$ be the number of communities in covers $C1$ and $C2$, respectively, the omega index $\omega$ is defined as [Gregory 2011; Havemann et al. 2011]
%
%\begin{equation}
%\omega(C_1, C_2) = \frac{\omega_u(C_1, C_2) - \omega_e(C_1, C_2)}{1 - \omega_e(C_1, C_2)}
%\label{eqn-omega}
%\end{equation}
%
%The unadjusted omega index $\omega_u$ is defined as
%
%\begin{equation}
%\omega_u(C_1, C_2) = \frac{1}{M} \sum\limits_{i=0}^{max(N_1,N_2)} \left\vert{s_i(C_1)\cap s_i(C_2)}\right\vert 
%\end{equation}
%
%where $M = n(n-1) /2$ represents the number of node pairs and $s_i(C)$ is the set of pairs that appear exactly $i$ times in a cover $C$. The expected omega index in the null model $\omega_e$ is given by
%
%\begin{equation}
%\omega_e(C_1, C_2) = \frac{1}{M^2} \sum\limits_{i=0}^{max(N_1,N_2)} \left\vert{s_i(C_1)}\right\vert \cdot \left\vert{s_i(C_2)}\right\vert 
%\end{equation}
%
%The subtraction of the expected value in Equation \ref{eqn-omega} takes into account agreements resulting from chance alone. The larger the omega index is, the better the matching is between two covers. A value of 1 indicates perfect matching. When there is no overlap, the omega index reduces to the ARI.

We evaluated the performance of our algorithm against the ground truth 
using {\it Omega Index} \cite{doi:10.1207/s15327906mbr2302_6}, 
which is the overlapping version of the Adjusted Rand Index (ARI) \cite{ARI_paper_1985}.
Intuitively, Omega Index measures the extent of agreement between two given sets of communities, by looking at node pairs that occur the same number of times (possibly none) in both.
We used three values for the parameter $c$ of our method: 0, 2, and 5. 
Recall that $c$ set to zero corresponds to picking only the largest clique for each node. 
As $c$ is increased, more and more large cliques (each of size at least $k$)
are considered for each node. 
We compare the performance of our method with that of CFinder\footnote{http://www.cfinder.org}, an implementation of CPM~\cite{cite-key}. We used the command line utility provided in the package for all experiments. For this study, we used a MacBook Pro running OS X v.10.9.2 with 2.66GHz Intel Core i7 processor with 2 cores, 256KB of L2 cache per core, 4MB of L3 cache and 8GB of main memory.

\input{results_application1}

%The results are shown in Table \ref{tab:applications1} and \ref{tab:applications2}. 

Table~\ref{tab:applications1} shows the experimental results we obtained.
The first three columns of the Table list the various parameters used to generate each test network. The fourth column lists the number of ground truth communities ($C(GT)$) in each network.  The remaining columns in the table show performance 
in terms of the number of communities detected ($C$), 
total number of shared nodes ($S$) and the Omega Index ($\Omega$) for 
CFinder and our method with different values for the parameter $c$.
In our experiments, for CFinder as well as all variants of our algorithm, 
we found that the value of $k=4$ gives the best Omega Index value relative 
to the ground truth. All results reported in Table~\ref{tab:applications1} are therefore
for $k=4$.

In general we observe that there is a close correlation between our method and CFinder
in terms of all three of the quantities $C$, $S$ and $\Omega$. It can be seen that as we increase the value of $c$ in our method, the Omega Index values get closer and closer to that of CFinder. For our algorithm run with $c=0$, the Omega Index is about 75$\%$ of that of CFinder. When run with $c$ = 2, it is about 92$\%$ and for $c$ = 5, it is about 99$\%$. When we increased the value of $c$ even further to 10, we observed that the Omega Index was almost identical to that obtained by CFinder. From this, one can see that we can get almost exactly the same results as the CPM method using our algorithm which uses only a small set of 
maximal cliques, as opposed to all the maximal cliques in the graph.

\input{results_application2}

Table~\ref{tab:applications2} shows the time taken by CFinder and our method 
run with $c$ = 0, 2 and 5. For our method, the table lists the total run time $\tau$ 
as well as the time $\tau_c$ spent on just the clique detection part and the ratio
${\tau_c}/{\tau}$ expressed in percents ($\tau_c$\%).
The remaining time $\tau - \tau_c$ is spent on building the clique-clique overlap matrix, eliminating cliques, component analysis and generating the communities.  As a side note,
we point out that our immediate goal in the implementation of these later phases has been quick experimentation, rather than efficient code, and therefore there is a very large room for improving the runtimes. This is also reflected by the numbers; one can see from the table that the average percentage of time our algorithm spends on clique-finding decreases as $c$ is increased; the quantity is about 30$\%$ when $c$ = 0 and about 16$\%$ when $c$ = 5. Yet, looking only at the total time taken in Table~\ref{tab:applications2}, and comparing CFinder and our algorithm run with $c$ = 5 (the case where the Omega Index values match most closely with CFinder), we see that our algorithm is at least 4$\times$ faster on average. When $c$ is set to 0 and 2, the mean speedups are 51$\times$ and 13$\times$ respectively. 
% Hence, the proportion of time the algorithm spends anything other than clique-detection progressively increases. 

%On the other hand, we noticed that CFinder spent most of its time in finding the cliques. 
Since the source code for CFinder is not publicly available, we were not able to measure exactly the proportion of time it spends on clique-finding. 
We suspect it constitutes a vast proportion of the total runtime.
%However, from our observation during the runs, we estimate this to be, on average, at least more than 95$\%$ of its total runtime. 
%If one assumes this to be 95$\%$, and also assuming the other parts of our algorithm (other than clique-finding) can be optimized to an equal proportion, our algorithm would be $\sim$28$\times$ for the $c$=5 case. 

%\subsection{Test on Real-world Networks}

\input{results_application3}

{\bf Test on Real-world Networks. } We also tested our method and CFinder on four of the real world graphs from our testbed in Section \ref{sec:experiments}---{\em cond-mat-2003}, {\em email-Enron}, {\em dictionary28} and {\em roadNet-CA}---and a user-interest-based graph generated using data collected from Facebook. We briefly explain here how this graph was generated.
Every user on Facebook has a {\it wall}, which is a the user's profile space that allows the posting of messages, often short or temporal notes or comments by other users. We generate a graph with the {\it walls} as vertices, and assign an edge between a pair of vertices, if there is at least one user who has commented on both walls. We assign edge weights proportional to the number of common users, as we consider this to be an indicator of the strength of the connection. A more elaborate explanation of the data collection method and network generation for the Facebook graph is discussed in \cite{dianapaper}. As this is a weighted graph, we used a threshold (of 0.009) to include only strong links, resulting in a network with 1144 vertices and 2561 edges.
%{\it walls}, and use this to formulate the network for our experiments.

\begin{figure}[h!]
  \centering
    %\includegraphics[width=1\textwidth]{communities_fb.pdf}
    \includegraphics[scale=0.4]{communities_fb_new.pdf}
    
\vspace{-15pt}
  \caption{Some Facebook communities detected by our algorithm.}
\label{fig-communities-fb}
\end{figure}
%\vspace{-10pt}

The results of our method for $c$ = 0 and 5, $k$ = 4, and CFinder for the case $k$ = 4 on all the five real-world graphs is shown in  Table~\ref{tab:applications3}. The table lists the number of communities found by each algorithm, total number of shared nodes, and the total time taken. For our algorithm, it also specifies the time spent on clique-finding. These graphs do not have any known community structure, so we were not able to measure the Omega Index values. For the graph {\em email-Enron}, CFinder was not able complete within 30 minutes. For the $c$ = 0 case, our algorithm comfortably outperforms CFinder, even in terms of total time, on average performing about 115$\times$ faster. For the $c$ = 5 case, the total time taken by our algorithm turns out to be higher for some cases, and lower for others. However, it should be noted that the time taken for clique finding is incomparably smaller than the post-clique-finding processing time. 
%If we make a previous assumption of 5$\%$ of the total time to which the post-clique-processing time can be reduced to, the speedup we gain would be on average, $\sim$576$\times$ faster for the $c$=0 case and $\sim$66$\times$ faster for the $c$=5 case.









%% (ref to supplementary info???).  
%
%
%We developed a very simple clique-based community detection algorithm using our heuristic as follows. We modified our heuristic such that it retains the largest clique containing each node. We use the heuristic instead of the exact algorithm because it is much faster and delivers near-optimal solution which is sufficient for the purpose of detecting communities. It is possible that we get duplicate cliques via different nodes,  
%and so we remove these. The resulting cliques are cohesively connected subgroups, and those are
%what our algorithm outputs as communities.
%
%%This is done by simply substituting Lines 3 and 4 of Algorithm \ref{alg:clqHeu}, with a simple routine that stores each clique in a preferred data structure. 
%
%
%%A detailed overview of community detection methods, and the significance and complexity involved in overlapping community findingcan be found in \cite{Fortunato_2010}.
%
%
%%\footnotetext{http://www.facebook.com}
%
%For experiments, we generated a user-interest-based network using data collected from 
%two widely used social media platforms: Facebook and Twitter.
%%\footnote[1]{http://www.facebook.com}  and Twitter \footnote[2]{http://www.twitter.com}. 
%Facebook {\it walls} and Twitter {\it profiles} are features in these platforms that provide a medium for businesses, groups and individuals to post content such as messages, promotions or campaigns. These features also engage other users by allowing them to reply or comment on the already posted content. We use users' comments on posts added on the Facebook {\it walls} as an indicator of their interests in the respective 
%{\it walls}, and use this to formulate the network for our experiments. The user comments and user information from specific {\it walls} are publicly available and collected using Facebook API\footnote[3]{http://developers.facebook.com/}. Similarly, for Twitter, we deduce users' interests by using their {\it tweets}. 
%A {\it tweet} is a message with up to 140 characters related to a particular Twitter {\it profile}. We use two kinds of {\it tweets}: {\it retweet}, which is a {\it tweet} made by a Twitter {\it profile} that gets tweeted again by another interested user, and {\it mentioned tweet}, which is a {\it tweet} made by an interested user regarding the Twitter profile. The publicly available user mentioned tweets, retweets of a Twitter profile, and information of users who tweeted on these profiles are collected using Twitter API\footnote[4]{https://dev.twitter.com/docs/}.
%
%
%
%With the collected data, we use the following technique to generate our user-interest-based network. From the gathered Facebook data, we calculate, for each {\it wall} $i$, the total number of unique users $u_i$ who have commented on it, and for each pair of {\it walls} $i, j$, the number of common users who have commented on both {\it walls} $c_{ij}$. The same procedure is carried out for Twitter {\it profiles}. We then construct an undirected graph $G = (V,E)$, where $V$ represents the {\it walls} or {\it profiles} and $E$ represents edges between them. We assign an edge between a pair of vertices, if there is at least one common user between them. The edge weight $w_{ij}$, which indicates the strength of the connection, is computed using the 
%Jacard index or similarity coefficient \cite{Leydesdorff} given by
%%\begin{equation}
%\[w_{ij} = \frac{c_{ij}}{u_i+u_j-c_{ij}}\]
%%\end{equation}
%
%It is clear from the above equation that the weight is between 0 and 1, a value closer to 1 implying the {\it walls}/{\it profiles} being more similar in terms of user interests.
%We then convert the graph to an unweighted graph by pruning edges whose weights are below a specified threshold, thus retaining only the links that indicate strong correlation. The choice of the threshold is subjective, and determines the size, number and quality of communities detected by our algorithm. 
%
%The weighted graph we formed using the Facebook data had 1144 vertices and 348,274, and that the Twitter graph had 1144 vertices and 204,131 edges. Since we look for the most cohesive subgroups, we set the threshold to a high number, that gave us fairly small communities with up to $\sim$15 vertices.
%
%
%%For our small experiment, we use data collected from Facebook\footnote[1]{http://www.facebook.com}. Every user on Facebook has a {\it wall}, which is a the user's profile space that allows the posting of messages, often short or temporal notes by other users. The user comments and user information from specific {\it walls} are publicly available and we collected them using Facebook API. We constructed a graph with the {\it walls} as vertices. Any two users who have commented on the same {\it wall} indicate a connection between the {\it walls}, and we form an edge between them. There could be many common users for each wall, and so we assigned edge weights by Jacard index or similarity coefficient \cite{Leydesdorff}. Once this is done for all {\it walls}, we retained only those edges which have weights above a chosen threshold, indicating a strong correlation. The threshold is a user's choice and decides both the size and the number of communities found.
%% If an edge already exists, we increase the edge weight by 1. Once this is done for all {\it walls}, the edge weights are normalized, and we retain only those edges which have edge weights above a chosen threshold (we use 0.01), indicating a strong correlation.
%
%%duplicate removal
%%We modified our heuristic to retain the largest maximum clique containing each node. 
%%This is done by simply substituting Lines 3 and 4 of Algorithm \ref{alg:clqHeu}, with a simple routine that stores each clique in a preferred data structure. 
%%The exact algorithm could have also been used instead of the heuristic for this purpose. We choose the heuristic since it is much faster and for this particular problem of community detection the accuracy of the size of cliques formed is not critical.


We also present some of the sports-related communities detected by our algorithm in the Facebook graph in Figure \ref{fig-communities-fb}, which is self-explanatory.
%We obtained a number of isolated communities similar to the one of {\it popular musicians}, and that of {\it internet corporations}. We also see communities that pertain to {\it MSNBC and its (news related) shows}, {\it news channels}, and {\it politics}. One can see that although the {\it news channels} and {\it MSNBC shows} communities are essentially separate, they share a common member, {\it MSNBC}, which is relevant to both. Similarly the {\it news channels} and {\it politics} communities share two nodes. One can see from that overlapping communities are a natural characteristic of real-world networks, which our algorithm helps in detecting.


%A few cautionary points need to be pointed out here. The figure represents only a small subset of the communities detected by our algorithm, which we decided to present here to illustrate the results of our algorithm. In reality, a large number of communities similar to the ones shown here were detected. Furthermore, the members in the communities also represent only a subset of nodes that belonged to that community, and we decided not to show the rest to favor clarity and simplicity. In order to improve readability, we have also decrypted the names of the nodes, which in reality were Facebook or Twitter handles of {\it walls} or {\it profiles}. The original handles lacked spaces in between words, had special characters such as underscore, or had additional terms, all of which we decided to leave out to help the reader better comprehend the names.

%As shown in Figure \ref{fig-communities-fb}, we obtained a number of isolated communities similar to the one of {\it popular singers}, and that of {\it internet corporations}. We also see communities that pertain to {\it MSNBC and its (news related) shows}, {\it news channels}, and {\it politics}. The point of this experiment is that our algorithm allows a node to be a member of more than one community and therefore helps detect overlapping communities. For instance, although the {\it news channels} and {\it MSNBC shows} communities are essentially separate, they share a common member, {\it MSNBC}, which is relevant to both. 
%
%A similar feature can be observed between the {\it news channels} and  {\it politics} communities
%where the two communities share two members. 
%Figure \ref{fig-communities-tw} shows the communities detected from the Twitter graph. 
%One can observe a very similar pattern there as well.
%%add from nature paper why this is significant. coexistence of their structural subunits 
%
%%\vspace{-20pt}
%\begin{figure}%[h!]
%  \centering
%    %\includegraphics[width=1\textwidth]{communities_tw.pdf}
%    \includegraphics[scale=0.25]{communities_tw.pdf}
%%\vspace{-30pt}
%  \caption{Some Twitter communities detected by our algorithm.}
%\label{fig-communities-tw}
%\end{figure}
%%\vspace{-10pt}
%

%As demonstrated by these experiments, the algorithm used here although rather elementary can be effective at detecting overlapping communities. Our algorithm, however, detects communities formed by cliques, which is a stringent requirement. Appropriate relaxations, such as the use of $k$-cores, is worth investigating and is one of the future lines of work we intend to pursue. 




%The immediate next thing to try would be to extend this to allow for clique-relaxations, such as $k$-core, $k$-plex \ref{Doreian1994267} etc. This can be done by merging the communities detected by our algorithm, which is one of the future lines of work we intend to pursue.


==> arXiv Submission/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%\vspace{-10pt}

We presented a new exact and a new heuristic algorithm for the maximum clique problem.
We performed extensive experiments on three broad categories of graphs comparing the 
performance of our algorithms to the algorithms by
Carraghan and Pardalos (CP) \cite{pardalos},
\"{O}sterg{\aa}rd ({\it cliquer}) \cite{ostergard}, Tomita et al. (MCQ, MCS) \cite{citeulike:7905505}\cite{walcom}, Konc and Jane\v{z}i\v{c} (MCQD) \cite{konc2007improved}, and Segundo et al. (BBMC)~\cite{SanSegundo}.
For DIMACS benchmark graphs and certain dense synthetic graphs ({\it rmat\_sd2}), our new exact algorithm performs comparably with the CP algorithm, but slower than the others. 
For large sparse graphs, both synthetic and real-world, our new algorithm runs
several orders of magnitude faster than the others. 
And its general runtime is observed to grow nearly linearly with the size of the graphs. 
The heuristic, which runs orders of magnitude faster than our exact algorithm and the others, delivers an optimal solution for 83\% of the test cases, and when it is sub-optimal, its accuracy ranges between 0.83 and 0.99 for the graphs in our testbed.
We also showed how the algorithms can be parallelized. Finally as a demonstration to the applications of clique finding algorithms, we presented a novel and efficient alternative based on our algorithms to the Clique Percolation Method \cite{cite-key}, to detect overlapping communities in networks. 

Maximum clique detection is often avoided by practitioners from being used as a component in 
a network analysis algorithm on the grounds of its NP-hardness. The results shown here suggest that this is not necessarily true, as maximum cliques can in fact be detected rather quickly for most real-world networks that are characterized by sparsity and other structures well suited for branch-and-bound type algorithms.

%Our comparison with existing algorithms is understandably not exhaustive. We have compared against a reasonable sample representatives with emphasis on those that have publicly available implementations. There are a number of algorithms that do not have publicly available implementation (e.g. \cite{walcom,AAAI101611}) and that would be interesting to compare against in future work. 

%Further, the MCQD implementation uses an adjacency matrix, whereas our algorithm uses an adjacency list to represent the graph. Although it is unlikely for the overall results to be drastically different with a change in the graph representation, it will be interesting to study to what degree the performance will change with
%the change in graph representation.
%The exact algorithm was in general  found to be less successful on relatively dense graphs.
%An interesting line of investigation would be to study ways to overcome this.
%The heuristic's performance is impressive as presented; still it is worthwhile
%to compare with other existing heuristics approaches such as \cite{heu1,heu2}. 
%Another line for future work would be to characterize the class(es) of graphs for which the heuristic is expected to return near-optimal solution.

==> arXiv Submission/experiments.tex <==
\section{Experimental Evaluation}
\label{sec:experiments}

We present in this section results comparing the performance of our algorithm
with other existing algorithms. Our experiments were performed on a Linux workstation running 64-bit Red Hat Enterprise Linux Server release 6.2 with a 2GHz Intel Xeon E7540 processor with 32GB of main memory. Our implementation is in C++, compiled using gcc version 4.4.6 with -O3 optimization.


\subsection{Test Graphs}

\begin{table}[!h]
%\small
\centering
\caption{Overview of real-world graphs in the testbed (UF, Pajek and Stanford datasets) and their origins.}
\label{tab:real-graphs}
\begin{tabular}{ll}
\hline \hline
{\bf Graph} & {\bf Description} \\ \hline \hline
{\it cond-mat-2003} \cite{Newman06042004} & A collaboration network of scientists posting preprints 
on \\ & the condensed matter archive at www.arxiv.org in the period \\ 
& between January 1, 1995 and June 30, 2003. \\
%The largest component of this network, which contains 27519 scientists, has been used by several authors as a test-bed for community-finding algorithms for large networks; see for example \cite{PhysRevE.72.027104}
{\it email-Enron} \cite{Leskovec:2005:GOT:1081870.1081893} & A communication network representing
email exchanges. \\
%This data was originally made public, and posted to the web, by the Federal Energy Regulatory Commission during its investigation. 
%Nodes are email addresses and there is a directed edge from \\ & node $i$ to node $j$ if at least one email is sent from $i$ to $j$. \\ \hline
%(In our experiments we ignore the directions and treat the graph as if it were undirected.)\\
%sent at least one email to address $j$, the graph contains a directed edge from $i$ to $j$. Note that non-Enron email addresses act as sinks and sources in the network as we only observe their communication with the Enron email addresses. 
{\it dictionary28} \cite{pajek2006} & Pajek network of words. \\ 
{\it Fault\_639} \cite{Ferronato20083922} & A structural problem discretizing a faulted gas reservoir with \\
& tetrahedral Finite Elements and triangular Interface Elements. \\
%& The Interface Elements are used with a Penalty formulation to simulate fault behavior. \\ \hline
%The problem arises from a 3D discretization with three displacement unknowns associated to each node of the grid. \\
{\it audikw\_1} \cite{Davis97theuniversity} & An automotive crankshaft model of TETRA elements. \\ 
{\it bone010} \cite{vanRietbergen199569} &
%Three-dimensional serial reconstruction techniques allow us to develop 
A detailed micro-finite element model of bones representing \\
& the porous bone micro-architecture. \\
%& Micro computed tomography (CT) is employed to make 3D high-resolution images. \\ \hline
% ($\sim$50 microns) of a bone. \\ \hline
%\\
%Then the 3D reconstruction is directly transformed into an equally shaped micro finite element model by simply converting all bone voxels to equally sized 8-node brick elements. This results in finite element (FE) models with a very large number of elements. \\
{\it af\_shell} \cite{Davis97theuniversity}  & A sheet metal forming simulation network. \\ 
{\it as-Skitter} \cite{Leskovec:2005:GOT:1081870.1081893} & An Internet topology graph from trace routes run daily in 2005. \\  %From several scattered sources to million destinations. %1.7 million nodes, 11 million edges. 
{\it roadNet-CA} \cite{Leskovec:2005:GOT:1081870.1081893} & A road network of California.
Nodes represent intersections \\ & and endpoints and edges represent the roads connecting them. \\  % \\ & intersections or endpoints. \\    \hline
{\it kkt\_power} \cite{Davis97theuniversity} & An Optimal Power Flow (nonlinear optimization) network. \\\hline
{\it foldoc} \cite{foldoc} & A searchable dictionary of terms related to computing. \\
{\it eatRS} \cite{eatRS} & The Edinburgh Associative Thesaurus, a set of word association \\ &
norms showing the counts of word association as collected \\ & from subjects. \\
{\it hep-th} \cite{hep-th-kdd}	& Citation data from KDD Cup 2003, a knowledge discovery and\\ & data mining
competition held in conjunction with the Ninth\\ & ACM SIGKDD Conference. \\
{\it patents} \cite{hall2001}	& Data set containing information on almost 3 million U.S.\\ & patents granted
between January 1963 and December 1999, and\\ & all citations made to
these patents between 1975 and 1999. 	\\
{\it days-all} \cite{corman2002}	& Reuters terror news network obtained from the CRA networks\\ & produced
by Steve Corman and Kevin Dooley at Arizona\\ & State University.	\\\hline
{\it roadNet-TX} \cite{Leskovec:2005:GOT:1081870.1081893}	& Road network of Texas.	\\
{\it amazon0601} \cite{leskovec2007}	& Amazon product co-purchasing network from June 1 2003. \\
{\it email-EuAll} \cite{leskovec2007-2}	& Email network from a EU research institution.	\\
{\it web-Google} \cite{web-google}	& Web graph released by Google in 2002 as a part of
Google\\ & Programming Contest.	\\
{\it soc-wiki-Vote} \cite{leskovec2010}	& Wikipedia who-votes-on-whom network.	\\
{\it soc-slashdot0902} \cite{Leskovec:2005:GOT:1081870.1081893}	& Slashdot social network from November 2008.\\
{\it cit-Patents} \cite{hall2001}	& Citation network among US Patents.	\\
{\it soc-Epinions1} \cite{richardson2003}	&	Who-trusts-whom network of Epinions.com. \\
{\it soc-wiki-Talk} \cite{leskovec2010}	&	Wikipedia talk (communication) network. \\
{\it web-berkstan} \cite{Leskovec:2005:GOT:1081870.1081893}	& Web graph of Berkeley and Stanford.	\\\hline\hline

\end{tabular}
\end{table}

Our testbed consists of 91 graphs, grouped in three categories:\\
\begin{enumerate*}[label=\textbf{\arabic*})]
\item {\bf Real-world graphs. } 
Under this category, we consider 10 graphs downloaded from the 
University of Florida (UF) Sparse Matrix Collection  \cite{Davis97theuniversity}, 5 graphs from Pajek data sets \cite{pajek2006}, and 10 graphs from the Stanford Large Network Dataset Collection \cite{stanford_dataset}.
The graphs originate
from various real-world applications. 
Table~\ref{tab:real-graphs} gives a quick overview of the graphs and their origins.\\


\item {\bf Synthetic Graphs. } 
In this category we consider 15 graphs generated using 
the R-MAT algorithm \cite{Chakrabarti:2006:GML:1132952.1132954}. The graphs
are subdivided in three categories depending on the structures they represent:\\

\begin{enumerate*}[label=\textbf{\alph*})]
\item {\bf Random graphs} (5 graphs) -- Erd\H{o}s-R\'{e}nyi random  graphs generated using R-MAT with the parameters (0.25, 0.25, 0.25, 0.25).  We denoted these with prefix {\it rmat\_er}.\\
\item {\bf Skewed Degree, Type 1 graphs} (5 graphs) -- graphs generated using R-MAT with the parameters (0.45, 0.15, 0.15, 0.25). These are denoted with prefix {\it rmat\_sd1}.\\
\item {\bf Skewed Degree, Type 2 graphs} (5 graphs) --  graphs generated using R-MAT with the parameters (0.55, 0.15, 0.15, 0.15). These are denoted with prefix {\it rmat\_sd2}.\\
\end{enumerate*}

\item {\bf DIMACS graphs. } 
This last category consists of 51 graphs selected from the Second DIMACS Implementation Challenge \cite{dimacs}. Among these, 5 graphs are considered for discussion in the next few sections, while the results for the rest are reported in Table \ref{tab:dimacs} in the Appendix.
\end{enumerate*}

The DIMACS graphs  are an established benchmark for the maximum
clique problem, but they are of rather limited size and variation. 
In contrast, the real-work networks included  in category 1 of the testset
and the synthetic (RMAT) graphs in category 2
represent a wide spectrum of large graphs posing varying degrees of difficulty for the algorithms. 
The {\it rmat\_er} graphs have {\it normal} degree distribution, whereas the {\it rmat\_sd1} and {\it rmat\_sd2} graphs have skewed degree distributions and contain many dense local subgraphs.
 The {\it rmat\_sd1} and {\it rmat\_sd2} graphs differ primarily in the magnitude of maximum vertex degree they contain; the {\it rmat\_sd2} graphs have much higher maximum degree. 
Table \ref{tab:struc-graphs} lists basic structural information (the number of vertices, 
number of edges and the maximum degree) about 45 of the test graphs (25 real-world, 15 synthetic and 5 DIMACS).

\input{graphs_properties}

\subsection{Algorithms for Comparison}
The algorithms we consider for comparison are the ones by: 
\begin{itemize}
\itemsep0em
\item Carraghan-Pardalos \cite{pardalos}. We used our own implementation of this algorithm.
\item \"{O}sterg{\aa}rd algorithm \cite{ostergard}. We used the publicly available {\it cliquer} source code \cite{cliquer}.
\item Konc and Jane\v{z}i\v{c} \cite{konc2007improved}. We used the code {\it MaxCliqueDyn} or MCQD, available at \\{\small \url{http://www.sicmm.org/~konc/maxclique/}}. Among the variants available in MCQD, we report results on MCQD+CS (which uses improved coloring and dynamic sorting), since it is the best-performing variant. The {\it MaxCliqueDyn} code was not capable of handling large input graphs and had to be aborted for many instances. For those that it successfully ran, we had to first modify the graph reader to make it able to handle graphs with multiple connected components.
\item Tomita and Seki (MCQ) \cite{citeulike:7905505}.
\item Tomita et al. (MCS) \cite{walcom}.
\item San Segundo et al. (BBMC) \cite{SanSegundo}.
\end{itemize}
For MCQ, MCS, and BBMC, we used the publicly available Java implementation, MCQ1, MCSa1, and BBMC1 respectively, by Prosser \cite{prosser2012}  available at {\small \url{http://www.dcs.gla.ac.uk/~pat/maxClique/}}. These implementations failed to run due to memory limitations in spite of making available 20 GB of memory for almost all (except two) of the larger data sets. Hence, timings are reported only for DIMACS graphs. 

In addition to comparing with the above mentioned algorithms, for the Pajek and Stanford data sets, we also provide comparison of the timing results of our algorithm with the maximal clique enumeration algorithm by Epstein \& Strash \cite{sea}. For this, we directly quote numbers published in \cite{sea}, and the results are listed in Table~\ref{tab:pajek_stanford-es} in the Appendix.
It should to be kept in mind that maximal clique enumeration in general is a harder problem than maximum clique finding, and that these experiments have been performed on different test environment. Therefore the runtime results should be understood in a sense qualitatively.


\subsection{Results}
\label{sec:exp-results}

\input{results_timings}
\input{new_timings}

Table~\ref{tab:timings} shows the size of the maximum clique ($\omega$) and the runtimes  of our exact algorithm (Algorithm 1) and the algorithms of Caraghan and Pardalos (CP), 
\"{O}sterg{\aa}rd ({\it cliquer}) 
and Konc and Jane\v{z}i\v{c}  (MCQD+CS) for all the graphs in the testbed except for 
the Pajek and Stanford test graphs;
results on the Pajek and Stanford graphs are presented in Table~\ref{tab:pajek_stanford}.
The last two columns in Table~\ref{tab:timings} show the results of our 
heuristic (Algorithm 2)---the size of the maximum clique 
returned ($\omega_{A_2}$)  and its runtime ($\tau_{A_2}$). 
The columns labeled $P1$, $P2$, $P3$ and $P5$ list the number of 
vertices/branches pruned in the respective pruning steps of Algorithm 1.
Data on Pruning 4 is omitted since that pruning is used by all of the algorithms compared in the table. The displayed pruning numbers have been rounded  (K stands for $10^3$, M for $10^6$ and B for $10^9$);
the exact numbers can be found in Table \ref{tab:prunings} in the Appendix.

In Table \ref{tab:timings}, the fastest runtime for each instance is indicated with boldface. 
An asterisk (*) indicates that an algorithm did not terminate within 25,000 seconds for a particular
instance. A hyphen (-) indicates that the publicly available implementation 
(the {\it MaxCliqueDyn} code) had to be aborted because the input graph was too large 
for the implementation to handle.
For the graph {\it rmat\_sd2\_5}, none of the algorithms computed the maximum clique size in 
a reasonable time; the entry there is marked with N, standing for  ``Not Known''.

We discuss in what follows our observations from this table
for the exact algorithm and the heuristic.

%\vspace{-10pt}
\subsubsection{Exact algorithms}
\label{sec:exp-exact}

As expected, our exact algorithm gave the same size of maximum clique as the other
three algorithms for all test cases. 
In terms of runtime,  its relative performance compared to the other three varied
in accordance with the advantages afforded by the various pruning steps.  

%{\bf Analysis of pruning steps.  }
Vertices that are discarded by Pruning 1 are skipped in the main loop of the algorithm, and the largest cliques containing them are not computed. Pruning 2 avoids re-computing previously computed cliques in the neighborhood of a vertex. In the absence of Pruning 1, the number of vertices pruned by Pruning 2 would be bounded by the number of edges in the graph (note that this is more than the total number of vertices in the graph). While Pruning 3 reduces the size of the input set on which the maximum clique is to be computed, Pruning 5 brings down the time taken to generate the intersection set in Line 12 of the subroutine. 
Pruning 4 corresponds to back tracking. Unlike Pruning steps 1, 2, 3 and 5, Pruning 4
is used  by all three of the other algorithms in our comparison. The primary strength of our algorithm is its ability to take advantage of pruning in multiple steps in a hierarchical fashion, allowing for opportunities for one or more of the steps to be triggered and positively impact the performance.

\begin{figure}
  \centering
    \includegraphics[scale=0.5]{pruned.pdf}
\caption{Number of ``pruned" vertices in the various pruning steps normalized
by the number of edges in the graph (in percents) for the UF collection graphs (we cut few bars reachining 140\% as their correspnding values are much higher).}
\label{fig-pruningplot}
\end{figure}


In Figure~\ref{fig-pruningplot} we show the number of vertices discarded by all
the  pruning steps of the exact algorithm normalized by the total number of edges
in a graph for the real-world graphs in Table \ref{tab:timings}. We cut few bars reachining
140\% as their correspnding values are much higher.
In the Appendix, we provide a complete tabulation of the raw numbers for the pruned vertices in all the steps for all the graphs in the testbed. It can be seen for these graphs pruning steps 2 and 5 in particular discard a large percentage of vertices, potentially resulting in large runtime savings. The general behavior of the pruning steps Pruning 1, 2, 3 and 5 for the synthetic graphs {\em rmat\_er} and {\em rmat\_sd1} was observed to be somewhat similar to that depicted in Figure~\ref{fig-pruningplot} for the real-world graphs. In contrast, for the DIMACS graphs, the number of vertices pruned in steps Pruning 1, 3 and 5 were observed to be zero; the numbers in the step Pruning 2 were non-zero but relatively modest.
%Since our new pruning steps hierarchically reduce the search space, one can expect a decreasing order of effect in the performance of Prunings 1, 2, 3 and 5, with Pruning 1 having the highest impact, and 5 the lowest. 


As a result  of the differences seen in the effects of the pruning steps, as discussed below,
the runtime performance of our algorithm (seen in Table \ref{tab:timings}) compared
to the other three algorithms varied in accordance with the difference in the structures represented 
by the different categories of graphs in the testbed.

{\bf Real-world Graphs. }
For most of the graphs in this category (Table \ref{tab:timings}), it can be seen that our algorithm runs several orders of magnitude faster than the other three, mainly due to the large amount of pruning the algorithm attained. These numbers also illustrate the great benefit of hierarchical pruning. 
For the graphs {\em Fault\_639}, {\em audikw\_1} and {\em af\_shell10}, 
Prunings 1, 3 and 5 have only minimal impact,
whereas Pruning 2 makes a big difference resulting in impressive runtimes. 
The number of vertices pruned in steps Pruning 1 and 3 varied among the 
graph {\em within} the
category, ranging from 0.001\% for {\it af\_shell} to a staggering 97\% for {\it as-Skitter} 
for the step Pruning 1. For the graphs in Table \ref{tab:pajek_stanford} as well, one can observe that our algorithm performs much better than the others.
%We observe that the relative speedup factor of our algorithm is the highest for
%the graphs with high maximum clique size and high maximum degree.
%as well. For instance, for as-Skitter reduction the search space is reduced dramatically due to pruning, and results in a very impressive performance.



{\bf Synthetic Graphs. }
For the synthetic graph types {\it rmat\_er} and {\it rmat\_sd1}, our algorithm clearly outperforms 
the other three by a few orders of magnitude in all cases. 
This is also primary due to the high number of vertices discarded by the new pruning steps. 
In particular, for {\it rmat\_sd1} graphs, between 30 to 37\% of the vertices are pruned just in the step Pruning 1. 
%The {\it rmat\_er} and the corresponding {\it rmat\_sd1} graphs have nearly equal number of vertices and edges, however, the timings of the {\it rmat\_er} graphs are relatively better because of the smaller size of the maximum clique and the smaller maximum degree. 
For the {\it rmat\_sd2} graphs, which have relatively larger maximum clique and higher maximum degree than the {\it rmat\_sd1} graphs, our algorithm is observed to be faster than 
CP but slower than {\em cliquer}. 

{\bf DIMACS Graphs. }
The runtime of our exact algorithm for the DIMACS graphs is 
in most cases comparable to that of CP and higher than that of {\it cliquer}
and MCQD+CS. 
%As can be seen from the Table  \ref{tab:timings}, 
For these graphs, only Pruning 2 was found to be effective, 
and thus the performance results agree with one's expectation. 
%We include in the Appendix timing results on a larger collection of DIMACS graphs. 
The timings on a much larger collection of DIMACS graphs are presented in Table \ref{tab:dimacs} in the Appendix.


It is to be noted that the DIMACS graphs are intended to serve as challenging test cases for the maximum clique problem, and graphs with such high edge densities and low vertex count are rare in practice. 
Most of these have between 20 to 1024 vertices with an average edge density of roughly 0.6, 
whereas, most real world graphs are often very large and sparse
as exemplified by the real-world graphs in our test bed.
Other good examples of instances with similar nature include Internet topology graphs \cite{Faloutsos:1999:PRI:316188.316229}, the web graph \cite{kumar:extracting}, and social network graphs \cite{Domingos:2001:MNV:502512.502525}.


%\vspace{-15pt}
\subsubsection{The Heuristic}
\label{sec:exp-heuristic}

It can be seen that our heuristic runs several orders of magnitude faster than our exact algorithm,
while delivering either optimal or very close to optimal solution.
It gave the optimal solution on 25 out of the 30 test cases.
On the remaining 5 cases where it was suboptimal, its accuracy ranges from 83\% to 99\% (on average 93\%).

Additionally, we run the heuristic by choosing a vertex randomly in Line \ref{maxDsel} of Algorithm \ref{alg:mClqHeu} instead of the one with the maximum degree. We observe that on average, the solution is optimal only for less than $40\%$ of the test cases compared to 83\% when selecting the maximum degree vertex.
%after three repetitions with different random seeds


\begin{SCfigure}
  \centering
    \includegraphics[width=7.8cm]{maxclqplot.pdf}
%%\vspace{-30pt}
  \caption{Runtime (normalized, mean) comparison between various algorithms. For each category of graph, first, all runtimes for each graph were normalized by the runtime of the slowest algorithm for that graph, and then the mean was calculated for each algorithm. Graphs were considered only if the runtimes for at least three algorithms was less than the 25,000 seconds limit set.}
\label{fig-timeplot}
\end{SCfigure}
%\vspace{-10pt}
%\vspace{-10pt}




\subsubsection{Further Analysis}
\label{sec:exp-further}

Figure~\ref{fig-timeplot} provides an aggregated visual summary of the runtime trends of
the various algorithms across the five categories of graphs in the testbed. 
%The bars in each category
%are created as follows. First the runtime for each algorithm for each graph in a category is divided by the runtime of the slowest algorithm for that graph. Then the mean of these is taken as a resut for the category. Values enter into the mean calculation when runtimes are available for
%at least three algorithms.


To give a sense of runtime growth rates, we provide in Figure~\ref{fig-runtimeplots} plots of the 
runtime of the new exact algorithm and the heuristic for the synthetic and real-world graphs 
in the testbed. In addition to the curves corresponding to the runtimes of the
{\em exact} algorithm and the {\em heuristic}, the figures also include a curve corresponding to
the number of {\em edges} in the graph divided by the clock frequency of the computing
platform used in the experiment. This curve is added to facilitate comparison between
the growth rate of the runtime of the algorithms with that of a linear-time (in the size of the graph) growth rate. 
It can be seen that the runtime of the heuristic by and large grows 
somewhat linearly with the size of a graph. The exact algorithm's runtime, which is orders of
magnitude larger than the heuristic, exhibited a similar growth behavior for these test-cases
even though its worst-case complexity suggests exponential growth in the general case. 


\begin{figure}
  \centering
    \includegraphics[scale=0.67]{compare_time_er.pdf}
    \includegraphics[scale=0.67]{compare_time_sd1.pdf}\\
    
    \includegraphics[scale=0.67]{compare_time_sd2.pdf}
    \includegraphics[scale=0.67]{compare_time_rw.pdf}
    
%%\vspace{-30pt}
 \caption{Run time plots of the new exact and heuristic algorithms. The third curve, labeled
 {\em edges}, shows the quantity number of edges in the graph divided by the clock 
 frequency of the computing platform used in the experiment. 
 }
\label{fig-runtimeplots}
\end{figure}



%Finally, we comment on our experience in using the 
%{\it MaxCliqueDyn} code.
%Unfortunately, the code failed to execute most of the  
%large instances in our testbed, including the majority of the RMAT and real-world instances,
%due to memory management issues in the code. 
%The entries in Table~\ref{tab:timings} marked with hyphen (-) show instances
%for which the code crashed.
%One of the few instance we were able to successfully run was {\it email-enron}.
%For it, the code took 4.91 seconds to compute the maximum clique 
%(using the same experimental setup), whereas our algorithm took only 0.998 seconds. 
%The memory issue also prevented us from do an extensive comparison with the other more recent algorithms 
%based on \cite{citeulike:7905505} and including \cite{Tomita:2007:EBA:1188122.1188130}, 
%since to our knowledge, there does not exist any other publicly available package 
%based on this algorithm. 
%On a related note, our attempts to run instances larger than the ones used in the experiments reported here on the
%the {\em cliquer}  package (\url{http://users.tkk.fi/pat/cliquer.html} \cite{cliquer}) failed because of similar memory leak issues. 
%This makes our code (available at \url{http://cucis.ece.northwestern.edu/projects/MAXCLIQUE/}) the only open source code,
%which has been tested to be capable of finding the maximum clique of large instances. Note that our code also
%includes a converter between two popular graph formats, DIMACS to/from matrix market.
%Even for the instances it eventually run successfully, we had to first make modifications to the graph reader
%to make it able to handle graphs with multiple connected components.
%{\it 
%The fixes and related discussion I had to do in the available source code of MaxCliqueDyn \cite{konc2007improved} is as follows:
%The graph reader fails to read large graphs specially when the graph contains disjoint vertices. 
%The reader tries to allocate memory based on the number of distinct vertices and it 
%assumes the number of vertices is equal to the number of distinct vertices (which could be much lower) as the package
%has mostly been developed keeping the densed small graphs in mind. 
%Because of this there code can't run for the massive sparse graphs as the vertex ID becomes higher
%than the number of vertices and therefore access invalid memory locations and gives segmentation fault.
%I guess the reason they do this is to reduce the required memory by the algorithm (as the reply from the author says,
%at every round it allocates memory equal to the number of vertices, and therefore eventually the expected space requirement
%could be O($n^2$)). We therefore fixed the problem 
%by disallowing the code to change the number of vertices to the number of dictinct vertices.
%After doing this we noticed that the reader is capable of loading larger sparse graphs, but the algorithm runs 
%for long time and incrementally asks huge memory and the job become killed at some point
%For example, we noticed when we run experiment on $Fault$ graph, its being killed when
%the allocated memory reaches 100 GB.
%}

%\input{applications}

%\vspace{-10pt}

==> arXiv Submission/graphs_properties.tex <==
\begin{table}[t]
%\small
%\scriptsize
\centering
\caption{Structural properties---the number of vertices $|V|$; the umber of edges $|E|$; and the maximum degree $\Delta$---of the graphs $G$ in the testbed.
The graphs on the left side are graphs from the UF collection, Pajek data sets, and Stanford Large Dataset collection. On the right are the   
RMAT graphs; and the DIMACS Challenge graphs.}  
\label{tab:struc-graphs}
%\begin{tabular}{l@{\hspace{2pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{8pt}}r@{\hspace{5pt}}|@{\hspace{5pt}}l@{\hspace{2pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{8pt}}r}
\begin{tabular}{l@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}|@{\hspace{5pt}}l@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r}

\toprule\toprule

$G$ & $|V|$ & $|E|$ & $\Delta$ & $G$ & $|V|$ & $|E|$ & $\Delta$ \\ \hline \hline
{\it cond-mat-2003} & 31,163	& 120,029	 & 202 &	{\it rmat\_sd1\_1} &    131,072 &    1,046,384 & 407           \\ \vspace*{\rowspace}
{\it email-Enron} & 36,692	 & 183,831 &	1,383  &	{\it rmat\_sd1\_2} &    262,144 &    2,093,552 &   558    \\ \vspace*{\rowspace}
{\it dictionary28} & 	52,652 &	89,038 &	38  &		{\it rmat\_sd1\_3} &    524,288 &    4,190,376 &    618  \\ \vspace*{\rowspace}
{\it Fault\_639} &    638,802 &    13,987,881 &    317 &  {\it rmat\_sd1\_4} &    1,048,576 &    8,382,821 &  802    \\ \vspace*{\rowspace}
{\it audikw\_1} &    943,695 &    38,354,076 &    344  &	 {\it rmat\_sd1\_5} &    2,097,152 &    16,767,728 &    1,069   \\ \vspace*{\rowspace}
{\it bone010} &    986,703 &    35,339,811 &    80 & 
{\it rmat\_sd2\_1} &    131,072 &    1,032,634 &    2,980        \\ \vspace*{\rowspace}
{\it af\_shell10} &    1,508,065 &    25,582,130 &    34 &  
{\it rmat\_sd2\_2} &    262,144 &    2,067,860 &    4,493      \\ \vspace*{\rowspace}
{\it as-Skitter} &    1,696,415 &    11,095,298 &  35,455 &
{\it rmat\_sd2\_3} &    524,288 &    4,153,043 &    6,342     \\ \vspace*{\rowspace}
{\it roadNet-CA} &    1,971,281 &    2,766,607 &    12 & 
{\it rmat\_sd2\_4} &    1,048,576 &    8,318,004 &    9,453      \\ \vspace*{\rowspace}	
{\it kkt\_power} &    2,063,494 &    6,482,320 &    95  &   
{\it rmat\_sd2\_5} &    2,097,152 &    16,645,183 &    14,066    \\

\midrule
\vspace*{\rowspace}

{\it foldoc}				&	13,356	&	91,470		&	728		&
{\it rmat\_er\_1} &    131,072 &    1,048,515 &    82 	 \\ \vspace*{\rowspace}  
{\it eatRS}				&	23,219	&	304,938		&	1090		&
{\it rmat\_er\_2} &    262,144 &    2,097,104 &    98 	 \\ \vspace*{\rowspace}
{\it hep-th}				&	27,240	&	341,923		&	2411		&
{\it rmat\_er\_3} &    524,288 &    4,194,254 &    94  	 \\ \vspace*{\rowspace}
{\it patents}			&	240,547	&	560,943		&	212		&
{\it rmat\_er\_4} &    1,048,576 &    8,388,540 &    97  	 \\ \vspace*{\rowspace}
{\it days-all}			&	13,308	&	148,035		&	2265		&
{\it rmat\_er\_5} &    2,097,152 &    16,777,139 &    102 	 \\
\midrule
\vspace*{\rowspace}

{\it roadNet-PA}			&	1,088,092	&	1,541,898		&	9		&
{\it hamming6-4} & 64 &    704 &    22 	 \\ \vspace*{\rowspace}
{\it roadNet-TX}			&	1,393,383	&	1,921,660		&	12		&
{\it johnson8-4-4} & 70 &    1,855 &    53   \\ \vspace*{\rowspace} 
{\it amazon0601}		&	403,394	&	2,247,318		&	2752		&
{\it keller4} &    171 &    9,435 &    124  \\ \vspace*{\rowspace}   
{\it email-EuAll}			&	265,214	&	364,481		&	7636		&
{\it c-fat200-5} &    200 &    8,473 &    86  \\ \vspace*{\rowspace} 
{\it web-Google}		&	916,428	&	4,322,051		&	6332		&
{\it brock200\_2} &    200 &    9,876 &    114 \\ \vspace*{\rowspace}
{\it soc-wiki-Vote}		&	8,297	&	100,762		&	1065		&
 &     &     &     \\ \vspace*{\rowspace}
{\it soc-slashdot0902}	&	82,168	&	504,230		&	2252		&
 &     &     &     \\ \vspace*{\rowspace}
{\it cit-Patents}			&	3,774,768	&	16,518,947	&	793		&
 &     &     &     \\ \vspace*{\rowspace}
{\it soc-Epinions1}		&	75,888	&	405,740		&	3044		&
 &     &     &     \\ \vspace*{\rowspace}
{\it soc-wiki-Talk}		&	2,394,385	&	4,659,565		&	100029	&
 &     &     &     \\ \vspace*{\rowspace}
{\it web-berkstan}		&	685,230	&	6,649,470		&	84230	&
 &     &     &     \\ 
\bottomrule\bottomrule
\end{tabular}
%\vspace{-6pt}
\end{table}


==> arXiv Submission/introduction.tex <==
\section{Introduction}
\label{sec:intro}
%\vspace{-6pt}

A clique in an undirected graph is a subset of vertices in which every two vertices
are adjacent to each other. The {\em maximum} clique problem seeks to find 
a clique of the largest possible size in a given graph.

The maximum clique problem, and the related {\em maximal} clique and 
clique {\em enumeration} problems, find applications in a wide variety of domains,
many intimately related to the World Wide Web. 
A few examples include:  
information retrieval \cite{Augustson:1970:AGT:321607.321608}, 
community detection in networks \cite{Fortunato_2010,cite-key,5586496}, 
spatial data mining \cite{wang2009order},
data mining in bioinformatics \cite{19566964},
disease classification based on symptom correlation \cite{Bonner:1964:CT:1662386.1662389}, 
pattern recognition \cite{1211348},
analysis of financial networks \cite{RePEc:eee:csdana:v:48:y:2005:i:2:p:431-443},
computer vision \cite{Horaud:1989:SCT:68871.68875}, and
coding theory \cite{brouwer}.
More examples of application areas can be found in 
\cite{Gutin2004,citeulike:4058448}.

To get a sense for how clique computation arises in the aforementioned contexts, 
consider a generic data mining or information retrieval problem. A typical objective
here is to retrieve data that are considered similar based on some metric. 
Constructing a graph in which vertices correspond to data items and 
edges connect similar items, a clique in the graph would then give a cluster of similar data. 

The maximum clique problem is NP-Hard \cite{Garey:1979:CIG:578533}.
Most exact algorithms for solving it employ some form of {\it branch-and-bound} approach. 
While branching systematically searches for all candidate solutions, bounding (also known as {\em pruning}) discards fruitless candidates based on a previously computed bound. 
The algorithm of Carraghan and Pardalos \cite{pardalos} is an early example of 
a simple and  effective branch-and-bound algorithm for the maximum clique problem.
%are \cite{Bomze99themaximum,pardalos}. 
More recently, \"{O}sterg{\aa}rd \cite{ostergard} introduced 
an improved algorithm and demonstrated its relative advantages via computational experiments. 
Tomita and Seki \cite{citeulike:7905505}, and later, Konc and Jane\v{z}i\v{c} \cite{konc2007improved}
use upper bounds computed using vertex coloring to enhance the branch-and-bound approach. 
%Sewell (1998) presented a maximum clique algorithm designed for dense graphs.
Other examples of branch-and-bound algorithms for the clique problem include 
the works of Bomze et al~\cite{Bomze99themaximum}, Segundo et al.~\cite{SanSegundo}
and Babel and Tinhofer~\cite{babel1990branch}.
Prosser~\cite{prosser2012} in a recent work compares various exact algorithms 
for the maximum clique problem. %An attractive feature of the algorithms of \cite{pardalos} and \cite{ostergard} is their simplicity in terms of ease of implementation. However, their runtimes could  be infeasible for very large graphs.

%only for graphs with up to a few thousand vertices and a corresponding number of edges. 
%Furthermore, both algorithms as well as 
%the algorithms from  \cite{citeulike:7905505} and \cite{konc2007improved}
%are inherently sequential and not naturally parallelizable. 
%The ease with which an algorithm can be parallelized is important 
%for handling large-scale graphs in emerging applications, where graphs with 
%millions (or more) vertices are quite common \cite{kumar:extracting}.

In this paper, we present a new exact branch-and-bound
algorithm for the maximum clique problem that employs 
several new pruning strategies in addition to those used in \cite{pardalos},
\cite{ostergard}, \cite{citeulike:7905505} and \cite{konc2007improved},
making it suitable for massive graphs.
%We also present a heuristic that is based on similar pruning techniques as the exact algorithm but runs much faster---the heuristic follows just one of the ``paths" in the search space, and as a result its complexity is nearly linear-time in the size of the graph, in contrast to the exact algorithm whose worst-case complexity is exponential. 
We run our algorithms on a large variety of test graphs and compare its performance with the
algorithms by Carraghan and Pardalos \cite{pardalos}, \"{O}sterg{\aa}rd \cite{ostergard}, Tomita et al. \cite{citeulike:7905505}\cite{walcom}, Konc and Jane\v{z}i\v{c} \cite{konc2007improved}, and Segundo et al.~\cite{SanSegundo}. 
We find our new exact algorithm to be up to orders of magnitude faster on large,
sparse graphs and of comparable runtime on denser graphs.
We also present a hew heuristic, which runs several orders of magnitude faster than the exact algorithm while providing solutions that are optimal or near-optimal for most cases. The algorithms are presented in detail in Section~\ref{sec:algorithms} and the experimental evaluations and comparisons are presented in Section~\ref{sec:experiments}. 

Both the exact algorithm and the heuristic are well-suited for parallelization.
We discuss a simple shared-memory parallelization and present performance 
results showing its promise in Section~\ref{sec:parallelization}. 
We also include (in Section~\ref{sec:applications})
an illustration on how the algorithms can be used as parts of a method
for detecting overlapping communities in networks.
We have made our implementations publicly available\footnote{\url{http://cucis.ece.northwestern.edu/projects/MAXCLIQUE/}}.
%The algorithms are discussed in detail in Section~\ref{sec:algorithms}.

%In Section~\ref{sec:experiments} we present an extensive experimental analysis comparing the performance of our algorithms with the algorithm of Carraghan and Pardalos \cite{pardalos}, the algorithm of \"{O}sterg\.{a}rd \cite{ostergard} and the algorithm of Konc and Jane\v{z}i\v{c} \cite{konc2007improved}.
%The workings of the latter three algorithms is reviewed in Section~\ref{sec:relatedwork}.

%Our testbed includes large-scale real-world graphs drawn from various application domains, large-scale synthetic graphs representing various structures, and DIMACS benchmark graphs.

% \cite{dimacs}, 
%the University of Florida collection, 
%\cite{Davis97theuniversity}, 
% \cite{Chakrabarti:2006:GML:1132952.1132954},
%\vspace{-10pt}



==> arXiv Submission/new_timings.tex <==
\begin{table}[tbh]
%\footnotesize
%\scriptsize
%\small
\centering
\caption{Comparison of runtimes of algorithms: \cite{ostergard} ({\it $\tau_{cliquer}$}), \cite{konc2007improved} ({\it $\tau_{MCQD+CS}$}), 
with that of our new exact algorithm ($\tau_{A1}$) for selected medium and large Pajek and Stanford data sets. 
An asterisk (*) indicates that the algorithm did not terminate within 
15,000 seconds for that instance. The column $\omega$ lists the maximum clique size in each graph, 
the column $\omega_{A_2}$ lists the clique size returned by our heuristic and the column
$\tau_{A_2}$ lists the heuristic's runtime.}
%Comparison between algorithms in \cite{pardalos} (CP), \cite{ostergard} (cliquer) and our new exact and
%heuristic algorithms.
%An asterisk (*) indicates that the algorithm did not terminate within 25,000 seconds for that problem instance.
%For the graph {\it rmat\_sd2\_5}, none of the algorithms computed the maximum clique size in a reasonable time;
%the entry is marked $N$, denoting ``Not Known''.
%The last two columns of the table show the numbers of vertices pruned in steps Pruning 1
%and Pruning 3 of Algorithm 1.} 
\label{tab:pajek_stanford}
%@{\hspace{5pt}}
%\begin{tabular}{l@{\hspace{10pt}}r@{\hspace{10pt}}r@{\hspace{10pt}}r@{\hspace{10pt}}r@{\hspace{10pt}}|@{\hspace{10pt}}r@{\hspace{10pt}}r}
%\begin{tabular}{lrrrrrr|rr}
%\begin{tabular}{l@{\hspace{6pt}}r@{\hspace{6pt}}|@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r}
\begin{tabular}{lr|rrr|rr}
\toprule\toprule
	&		&			&	$\tau_{MCQD}$	&		&		&		\\
$G$	&	$\omega$	&	$\tau_{cliquer}$	&	$_{+CS}$	&	$\tau_{A1}$	&	$\omega_{A2}$	&	$\tau_{A2}$	\\ \hline \hline
{\it foldoc}	&	9	&	2.23	&	0.58	&	0.05	&	9	&	$<$0.01	\\
{\it eatRS}	&	9	&	7.53	&	1.86	&	1.81	&	9	&	1.80	\\
{\it hep-th}	&	23	&	9.43	&	2.43	&	4.48	&	23	&	0.06	\\
{\it patents}	&	6	&	2829.48	&	239.66	&	0.13	&	6	&	0.03	\\
{\it days-all}	&	28	&	2.47	&	0.59	&	75.37	&	21	&	0.05	\\
\midrule
{\it roadNet-TX}	&	4	&	*	&	*	&	0.26	&	4	&	0.04	\\
{\it amazon0601}	&	11	&	3190.11	&	717.99	&	0.20	&	11	&	0.30	\\
{\it email-EuAll}	&	16	&	943.74	&	270.67	&	0.92	&	14	&	0.06	\\
{\it web-Google}	&	44	&	10958.68	&	*	&	0.35	&	44	&	0.6	\\
{\it soc-wiki-Vote}	&	17	&	0.89	&	0.24	&	4.31	&	14	&	0.02	\\
{\it soc-slashdot0902}	&	27	&	88.38	&	23.63	&	25.54	&	22	&	0.06	\\
{\it cit-Patents}	&	11	&	2.47	&	*	&	19.99	&	10	&	4.15	\\
{\it soc-Epinions1}	&	23	&	73.85	&	19.95	&	15.01	&	19	&	0.06	\\
{\it soc-wiki-Talk}	&	26	&	*	&	*	&	6885.13	&	18	&	0.45	\\
{\it web-berkstan}	&	201	&	6416.61	&	*	&	44.70	&	201	&	32.03	\\
	\bottomrule\bottomrule
\end{tabular}
\end{table}


==> arXiv Submission/parallelization.tex <==
\section{Parallelization}
\label{sec:parallelization}

%The ease with which an algorithm can be parallelized and its performance is important for handling large-scale graphs in emerging applications, where graphs with millions (or more) vertices have become quite common. 

 We demonstrate in this section how our exact algorithm can be parallelized and show performance results
on a shared-memory platform. The heuristic can be parallelized following a similar procedure.

%We here describe the parallelization procedure for both shared and distributed memory architecture. 
As explained in Section \ref{sec:algorithms}, the $i$th iteration of the {\em for} loop in the exact algorithm (Algorithm 1) computes the size of the largest clique that contains the vertex $v_i$. Since our algorithm does not impose any specific order in which vertices have to be processed, these iterations can in principle be performed concurrently. During such a concurrent computation, however, different processes might discover maximum cliques of different sizes---and for the pruning steps to be most effective, the current globally largest maximum clique size needs to be communicated to all processes as soon as it is discovered. In a shared-memory programming model, the global maximum clique size can be stored as a shared variable accessible to all the processing units, and its value can be updated by the relevant processor at any given time. In a distributed-memory setting, more care needs to be exercised to keep the communication cost low. 
%For the distributed case, the effects of pruning could, however, be tolerably compromised in order to enable the parallel computation. This can, for example, be done by using the most recent value of the maximum clique size for pruning, and updating this value by having synchronization steps at regular intervals.

\begin{figure}[!h]
  \centering
    \includegraphics[scale=0.21]{parallel_realworld_timing.pdf}
    \includegraphics[scale=0.21]{parallel_realworld_speedup.pdf}
    \includegraphics[scale=0.21]{parallel_other_timing.pdf}
    \includegraphics[scale=0.21]{parallel_other_speedup.pdf}
    
%%\vspace{-30pt}
 \caption{Performance (timing and speedup plots) of shared-memory parallelization on graphs in the test-bed. The top set of figures show performance on the real-world graphs, whereas the bottom set show results for the RMAT graphs. Graphs whose sequential runtime is less than 5 seconds were omitted.}
\label{fig-parallel_perf}
\end{figure}

We implemented a shared-memory parallelization based on the procedure described above using OpenMP. Since the global value of the maximum clique is shared by all processing units, we embed the step that updates the maximum clique, i.e. Line \ref{critical} of Algorithm \ref{alg:mClq}, into a {\it critical} section (an OpenMP feature that enforces a lock, thus allowing only one thread at a time to make the update). Further, we use dynamic load scheduling, since different vertices might return different sizes of maximum clique resulting in different work loads.
%, so would work best for our case.

We performed experiments on the same graphs listed in the testbed described in Section \ref{sec:experiments}. For these, we used a Linux workstation 
%running 64-bit version Red Hat Enterprise Linux Server release 6.2 
with six 2.00GHz Intel Xeon E7540 processors. Each processor has six cores, each with 32KB of L1 and 256KB of L2 cache, and each processor shares an 18MB L3 cache.  
%Implementation was in C++ using OpenMP and compiled with gcc (version 4.4.7) using the -O3 optimization flag.



Figure \ref{fig-parallel_perf} shows the timings and speedups we obtained for the real-world and RMAT graphs separately. We omitted graphs whose sequential runtimes were less than 5 seconds as they were too low to measure and do meaningful assessment of parallelization performance. For most of the real-world graphs, one can see from the figure that we obtained near-linear scaling of runtimes and speedups when up to 16 threads are used. The only exception is the graph 
{\emph as-Skitter}. The relatively poorer scaling there is likely due to the fact that the instance has a relatively large maximum clique, and hence the core (thread) which computes it spends relatively large amount of time computing it while other cores (threads) which have completed their processing of the remaining vertices remain idle. 
For the other instances of the real-world graphs, the maximum speedup we obtained 
while using 32 cores/threads is around 22$\times$. 

For the RMAT graphs, it can be seen that the scaling of the runtime and speedups vary with the structures (RMAT parameters) of the instances. We observed super-linear speedups for a couple of the instances, which
happens as a result of some unfruitful searches in the branch-and-bound procedure being discovered early
as a result of parallel processing. This phenomenon is better exploited and more fully explored in other works in the literature such as  \cite{a6040618}.
For the other instances, the algorithm scales fairly well up to 8 threads, and begins to
degrade thereafter. The speedups we obtained range between 6$\times$  to 20$\times$ when 32 threads are used.





%The effects of pruning could, although, be tolerably compromised in order to enable the parallel computation by allowing the processors to use the locally computed maximum clique value as the lower bound for pruning until regular synchronization steps, during which it is updated to the global value of the maximum clique across all processors.

%When done in parallel, the for loop in Algorithm \ref{alg:mClq} can be distributed among different $p$ computational units which can compute different values for $max$ in parallel. In the next step, a reduce operation can be used to find the maximum of the $p$ values.

%In this section we show the results of parallelization of our exact algorithm on shared memory architectures. In our algorithm, there is no dependency or strict order in which the vertices have to be computed unlike other previous algorithms. The sizes of the largest cliques containing different vertices can be computed mostly independently, and thus can be done in parallel by different computational units.


%\begin{figure}
%        \centering
%        \begin{subfigure}[b]{0.5\textwidth}
%                \includegraphics[width=\textwidth]{parallel_realworld_timing.pdf}
%                \caption{Timing results}
%                \label{fig:timing_realworld}
%        \end{subfigure}%
%        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
%          %(or a blank line to force the subfigure onto a new line)
%        \begin{subfigure}[b]{0.5\textwidth}
%                \includegraphics[width=\textwidth]{parallel_realworld_speedup.pdf}
%                \caption{Speedup results}
%                \label{fig:speedup_realworld}
%        \end{subfigure}
%        \caption{Performance of shared-memory parallelization on real-world graphs}\label{fig:animals}
%\end{figure}
%
%
%\begin{figure}
%        \centering
%        \begin{subfigure}[b]{0.5\textwidth}
%                \includegraphics[width=\textwidth]{parallel_other_timing.pdf}
%                \caption{Timing results}
%                \label{fig:timing_realworld}
%        \end{subfigure}%
%        ~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
%          %(or a blank line to force the subfigure onto a new line)
%        \begin{subfigure}[b]{0.5\textwidth}
%                \includegraphics[width=\textwidth]{parallel_other_speedup.pdf}
%                \caption{Speedup results}
%                \label{fig:speedup_realworld}
%        \end{subfigure}
%        \caption{Performance of shared-memory parallelization on real-world graphs}\label{fig:parallel_perf}
%\end{figure}
%







==> arXiv Submission/relatedwork.tex <==
%\section{The Carraghan-Pardalos and  \"{O}sterg\.{a}rd Algorithms}
\section{Related Previous Algorithms}
\label{sec:relatedwork}
%\vspace{-6pt}

Given a simple undirected graph $G$, the maximum clique can clearly be obtained by enumerating 
{\em all} of the cliques present in it and picking the largest of them.
Carraghan and Pardalos \cite{pardalos} introduced a simple-to-implement
algorithm that avoids enumerating all cliques and instead
works with a significantly reduced partial enumeration.
The reduction in enumeration is achieved via 
a {\em pruning} strategy which reduces the search space tremendously.
The algorithm works by
performing at each step $i$, a {\em depth first search} from vertex $v_i$, 
where the goal is to find the largest clique containing the vertex $v_i$.
At each {\em depth} of the search, the algorithm compares the number of remaining
vertices that could potentially constitute a clique containing vertex $v_i$
against the size of the largest clique encountered thus far.
If that number is found to be smaller, the algorithm backtracks (search is pruned).

\"{O}sterg{\aa}rd \cite{ostergard} devised an algorithm that incorporated an additional 
pruning strategy to the one by Carraghan and Pardalos.
The opportunity for the new pruning strategy is created by {\em reversing} the order in which the search is done by
the Carraghan-Pardalos algorithm. This allows for an additional pruning with the help of
some auxiliary book-keeping. 
Experimental results in \cite{ostergard} showed that the \"{O}sterg{\aa}rd
algorithm is faster than the Carraghan-Pardalos algorithm on random and 
DIMACS benchmark graphs \cite{dimacs}.
However, the new pruning strategy used in this algorithm is intimately tied to the order in which vertices are processed, introducing an inherent sequentiality into the algorithm.
% which renders it unsuitable for easy parallelization.

A number of existing branch-and-bound algorithms for maximum clique
also use a vertex-coloring of the graph to obtain an upper bound on the maximum clique. 
%A {\em vertex-coloring} of a graph is an assignment of colors to vertices such that  a pair of adjacent vertices receive different colors. Clearly, the number of colors used gives  an upper bound on the maximum clique of the graph, which can be used to reduce the search space. 
A popular and recent method based on this idea is 
the MCQ algorithm of Tomita and Seki \cite{citeulike:7905505}. 
More recently, Konc and Jane\v{z}i\v{c} \cite{konc2007improved} presented 
an improved version of MCQ, known as MaxCliqueDyn (with the variants MCQD and MCQD+CS), that involves the use of tighter, computationally more expensive upper bounds 
applied on a fraction of the search space. Another improved version of MCQ is BBMC by San Segundo et al. \cite{SanSegundo}, which makes use of bit strings to sort vertices in constant time as well as to compute graph transitions and bounds efficiently.

%They present two variations - 1) MCQ with improved 
%approximate coloring algorithm ColorSort (MCQ+CS) and 2) MCQ with improved coloring and dynamic sorting 
%of vertices (MCQD+CS)). The authors observe the latter to outperform MCQ on random and DIMACS benchmark graphs.

%\vspace{-12pt}


==> arXiv Submission/results_application1.tex <==
\begin{table}[!h]

\footnotesize
%\scriptsize
\small
\centering
\caption{Results of communities detected using our new method and CFinder on LFR benchmarks \cite{2008PhRvE..78d6110L}. 
All networks have $n$ = 1000 nodes, and the parameters used to generate the netwroks are listed in the first three columns: $\mu$ is the mixing parameter, $O_m$ is the number of communities each overlapping node is assigned to $O_n$ is the fraction of overlapping nodes. $C(GT)$ is the number of communities in the input graph (ground truth). $C$ denotes the number of communities, $S$ the number of shared nodes, and $\Omega$ the omega index. }
\label{tab:applications1}
%\begin{tabular}{l@{\hspace{6pt}}r@{\hspace{6pt}}|@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}|@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}|@{\hspace{6pt}}r@{\hspace{6pt}}r}

%\begin{tabular}{ c@{\hspace{4pt}}  c@{\hspace{2pt}}  c | @{\hspace{2pt}}c@{\hspace{2pt}} || c@{\hspace{2pt}}  c@{\hspace{2pt}}  c@{\hspace{4pt}} | c@{\hspace{3pt}}  c@{\hspace{3pt}}  c@{\hspace{3pt}} | c@{\hspace{3pt}}  c@{\hspace{3pt}}  c@{\hspace{3pt}}  | c@{\hspace{3pt}}  c@{\hspace{3pt}} c@{\hspace{3pt}}  }
\begin{tabular}{ c c c c || c@{\hspace{3pt}} c@{\hspace{3pt}} c@{\hspace{3pt}} | c c c | c c c | c c c }
\toprule\toprule
%	&  			& 			& 			&  		& 	CFinder	&			&		&Our Method	&			&		&	Our Method&			&		&Our Method	&		\\
	&  			& 			& 			&  		& 	CFinder	&	&	\multicolumn{9}{|c}{Our Method}			\\
%\hline
	&  			& 			& 			&  		& 		&		&	\multicolumn{3}{c}{$c=0$}&	\multicolumn{3}{c}{$c=2$}	&		\multicolumn{3}{c}{$c=5$}		\\
\hline
$\mu$&	$O_m$	&	$O_n$	&	$C(GT)$	&	$C$	&	$S$	&	$\Omega$	&	$C$	&	$S$		&	$\Omega$	&	$C$	&	S		&	$\Omega$	&	$C$	&	$S$	&	$\Omega$	\\
\hline\hline
0.1	&	2	&	10\%	&	34	&	37	&	55	&	0.842	&	60	&	64	&	0.758	&	49	&	76	&	0.825	&	40		&	59	&	0.840	\\
0.1	&	2	&	50\%	&	44	&	62	&	153	&	0.402	&	87	&	116	&	0.280	&	83	&	158	&	0.363	&	68		&	158	&	0.395	\\
0.1	&	8	&	10\%	&	51	&	58	&	30	&	$\sim$0.0	&	76	&	46	&	$\sim$0.0	&	65	&	39	&	$\sim$0.0	&	61		&	35	&	$\sim$0.0	\\
0.1	&	8	&	50\%	&	130	&	74	&	68	&	0.030	&	74	&	56	&	0.020	&	79	&	66	&	0.028	&	79		&	72	&	0.030	\\
0.3	&	2	&	10\%	&	35	&	50	&	53	&	0.612	&	69	&	67	&	0.461	&	64	&	73	&	0.577	&	55		&	60	&	0.605	\\
0.3	&	2	&	50\%	&	44	&	60	&	95	&	0.193	&	92	&	93	&	0.109	&	85	&	102	&	0.152	&	77		&	106	&	0.169	\\
0.3	&	8	&	10\%	&	48	&	64	&	35	&	0.304	&	79	&	59	&	0.239	&	74	&	55	&	0.293	&	69		&	46	&	0.301	\\
0.3	&	8	&	50\%	&	142	&	57	&	43	&	0.019	&	58	&	46	&	0.013	&	61	&	49	&	0.017	&	59		&	45	&	0.018	\\
\bottomrule\bottomrule
\end{tabular}

\end{table}


==> arXiv Submission/results_application2.tex <==
\begin{table}[!h]

\footnotesize
%\scriptsize
\small
\centering
\caption{Timing results of our new method and CFinder on the LFR benchmarks. All networks have $n$ = 1000 nodes, and the parameters used to generate the graphs are given by the first three columns: $\mu$ is the mixing parameter,  $O_m$ is the number of communities each overlapping node is assigned to and $O_n$ is
the fraction of overlapping nodes, $\tau_c$ is the time spent (in seconds) on computing the cliques, $\tau$ is the total time (in seconds), and $\tau_c\%$ is the percentage of time spent for clique computation. }
\label{tab:applications2}
%\begin{tabular}{l@{\hspace{6pt}}r@{\hspace{6pt}}|@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}|@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}|@{\hspace{6pt}}r@{\hspace{6pt}}r}

%\begin{tabular}{ c@{\hspace{4pt}}  c@{\hspace{2pt}}  c | @{\hspace{2pt}}c@{\hspace{2pt}} || c@{\hspace{2pt}}  c@{\hspace{2pt}}  c@{\hspace{4pt}} | c@{\hspace{3pt}}  c@{\hspace{3pt}}  c@{\hspace{3pt}} | c@{\hspace{3pt}}  c@{\hspace{3pt}}  c@{\hspace{3pt}}  | c@{\hspace{3pt}}  c@{\hspace{3pt}} c@{\hspace{3pt}}  }
\begin{tabular}{ c c c || c | c c c | c c c | c c c }
\toprule\toprule
 	&  		& 		&	CFinder	&			\multicolumn{9}{c}{Our Method}			\\
 	&  		& 		&			&			\multicolumn{3}{c}{$c=0$}				&		\multicolumn{3}{c}{$c=2$}	&	\multicolumn{3}{c}{$c=5$}				\\
\hline
$\mu$&$O_m$	&$O_n$	&	$\tau$	&	$\tau_c$	&	$\tau$	&$\tau_c\%$	&	$\tau_c$	&	$\tau$	&$\tau_c\%$	&	$\tau_c$	&	$\tau$	&$\tau_c\%$	\\
\hline\hline
0.1	&	2	&	10\%	&	0.913	&	0.005	&	0.031	&	17.3\%	&	0.025	&	0.255	&	9.7\%	&	0.050	&	0.912	&	5.5\%	\\
0.1	&	2	&	50\%	&	0.855	&	0.004	&	0.016	&	22.0\%	&	0.010	&	0.089	&	10.8\%	&	0.017	&	0.254	&	6.8\%	\\
0.1	&	8	&	10\%	&	0.732	&	0.004	&	0.025	&	17.4\%	&	0.012	&	0.159	&	7.4\%	&	0.024	&	0.550	&	4.4\%	\\
0.1	&	8	&	50\%	&	0.358	&	0.002	&	0.005	&	42.8\%	&	0.006	&	0.016	&	36.1\%	&	0.011	&	0.042	&	26.7\%	\\
0.3	&	2	&	10\%	&	0.592	&	0.004	&	0.013	&	26.0\%	&	0.011	&	0.090	&	11.8\%	&	0.027	&	0.321	&	8.3\%	\\
0.3	&	2	&	50\%	&	0.434	&	0.002	&	0.006	&	38.1\%	&	0.006	&	0.024	&	27.2\%	&	0.013	&	0.068	&	18.4\%	\\
0.3	&	8	&	10\%	&	0.472	&	0.003	&	0.011	&	25.7\%	&	0.008	&	0.064	&	12.5\%	&	0.016	&	0.205	&	7.6\%	\\
0.3	&	8	&	50\%	&	0.326	&	0.002	&	0.005	&	50.0\%	&	0.006	&	0.011	&	54.9\%	&	0.017	&	0.034	&	51.3\%	\\\bottomrule\bottomrule
\end{tabular}

\end{table}


==> arXiv Submission/results_application3.tex <==
\begin{table}[!h]

\footnotesize
%\scriptsize
\small
\centering
\caption{Results of our new algorithm and CFinder on three real-world graphs from Table \ref{tab:struc-graphs} and one additional graph generated using data collected from Facebook. The structural properties of the former three graphs are listed in Table \ref{tab:struc-graphs}. The Facebook graph has 1144 vertices and 2561 edges after thresholding. $C$ is the total number of communities found, $S$ is the total number of shared nodes, 
$\tau_c$ is the time spent (in seconds) on computing the cliques, and $\tau$, the total time (in seconds). A '-' denotes the algorithm did not complete in 30 minutes.}
\label{tab:applications3}
%\begin{tabular}{l@{\hspace{6pt}}r@{\hspace{6pt}}|@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}|@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}|@{\hspace{6pt}}r@{\hspace{6pt}}r}

%\begin{tabular}{ c@{\hspace{4pt}}  c@{\hspace{2pt}}  c | @{\hspace{2pt}}c@{\hspace{2pt}} || c@{\hspace{2pt}}  c@{\hspace{2pt}}  c@{\hspace{4pt}} | c@{\hspace{3pt}}  c@{\hspace{3pt}}  c@{\hspace{3pt}} | c@{\hspace{3pt}}  c@{\hspace{3pt}}  c@{\hspace{3pt}}  | c@{\hspace{3pt}}  c@{\hspace{3pt}} c@{\hspace{3pt}}  }
\begin{tabular}{ l || c c c | c c c c | c c c c }
\toprule\toprule
 					&  		\multicolumn{3}{c}{CFinder}			&		\multicolumn{8}{|c}{Our Method}			\\
 					&  		\multicolumn{3}{c}{}			&		\multicolumn{4}{|c}{$c=0$}			&	\multicolumn{4}{c}{$c=5$}		\\
\hline
$Name$				&	$C$	&	S	&$\tau$		&	$C$	&	$S$	&	$\tau_c$	&	$\tau$	&	C	&	S	&$\tau_c$		&	$\tau$	\\
\hline\hline
{\em cond-mat-2003}		&	4132	&	5180	&	68.46	&	3081	&	3937	&	0.130	&	14.000	&	3070	&	4460	&	0.917	&	417.151	\\
{\em email-Enron}		&	-	&	-	&	-		&	3947	&	4229	&	0.096	&	7.505	&	2518	&	3899	&	0.819	&	353.236	\\
{\em dictionary28}		&	3675	&	4308	&	9.67		&	2185	&	1799	&	0.040	&	1.132	&	3222	&	4154	&	0.300	&	95.596	\\
{\em roadNet-CA}		&	41	&	0	&	312.21	&	42	&	0	&	1.788	&	2.290	&	42	&	0	&	13.287	&	21.620	\\
{\em facebook}	&	29	&	29	&	3.42		&	38	&	46	&	0.002	&	0.011	&	19	&	27	&	0.023	&	0.252	\\
\bottomrule\bottomrule
\end{tabular}

\end{table}


==> arXiv Submission/results_timings.tex <==
\begin{table}[!hbt]

%\footnotesize
%\scriptsize
\small
\centering
\caption{Comparison of runtimes (in seconds) of algorithms {\it CP}~\cite{pardalos}, 
 {\it cliquer}~\cite{ostergard},  MCQD+CS~\cite{konc2007improved} and
and our new exact algorithm (${A_1}$) for the graphs in the testbed. An asterisk (*) indicates that the algorithm did not terminate within 25,000 seconds for a particular
instance. A hyphen (-) indicates that the publicly available implementation we used could not handle this instance due to its large size. Columns $P1$, $P2$, $P3$ and $P5$ list the number of vertices/branches pruned in steps Pruning 1, 2, 3 and 5 of our exact algorithm (K stands for the quantity $10^3$, M for $10^6$ and B for $10^9$). 
The column $\omega$ (second column) lists the maximum clique size in each graph, 
the column $\omega_{A_2}$ lists the clique size returned by our heuristic and the column
$\tau_{A_2}$ lists the heuristic's runtime.}
\label{tab:timings}
\begin{tabular}{l@{\hspace{6pt}}r@{\hspace{6pt}}|@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}r@{\hspace{6pt}}|@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}r@{\hspace{4pt}}|@{\hspace{6pt}}r@{\hspace{6pt}}r}

\toprule\toprule
           &  & & &  $\tau_{MCQD}$ & &	&	&	&	&& \\
Graph           	& $\omega$ & $\tau_{CP}$    & $\tau_{cliquer}$  & $_{+CS}$  &  $\tau_{A_1}$		& 	$P1$ 		&	$P2$		& 	$P3$ 		&	$P5$		 & $\omega_{A_2}$ &  $\tau_{A_2}$ \\
\hline \hline
%Graph 			& $\omega$ & $\tau_{CP}$ 	& $\tau_{cliquer}$	& $\tau_{MCQD+CS}$	& $\tau_{new-exact}$ & $\omega_{new-heuristic}$& $\tau_{new-heuristic}$\\ \hline \hline
%\vspace{-4pt} \\
%				& 		& 		 		& 				& $_{-exact}$ 	 	& $_{-heuristic}$ 	& $_{-heuristic}$	\\ \hline \hline
{\it cond-mat-2003} 	& 	25 	& 	4.87 			&  	11.17		&	2.41		&	{\bf 0.011}		& 	29K 			&	48K			&	6,527 		& 	17K			&	25 		& 	$<$0.01 	\\
{\it email-Enron} 	& 	20 	& 	7.01			& 	15.08 		&	3.70		& 	{\bf 0.998}		& 	32K 			&	155K		&	4,060 		& 	8M			&	18 		& 	0.26	\\ %8,835,739	
{\it dictionary28} 	& 	26 	& 	7.70	 		&	32.74 		&	7.69		&	{\bf $<$0.01}	& 	52K			& 	4,353		&	2,114		& 	107			&	26 		&	$<$0.01	\\	
{\it Fault\_639}		&	18	&	14571.20		&	4437.14		&	-		&	{\bf 20.03}		&	36			&	13M			&	126			&	1,116		&	18		&	5.80 		\\
{\it audikw\_1}		&	36	&	*			&	9282.49		&	-		&	{\bf 190.17}	&	4,101		&	38M			&	59K			&	721K		&	36		&	58.38 	\\
{\it bone010}		&	24	&	*			&	10002.67		&	-		&	{\bf 393.11}	&	37K			&	34M			&	361K		&	44M			&	24		&	24.39 	\\ %43,991,787
{\it af\_shell10}		&	15	&	*			&	21669.96		&	-		&	{\bf 50.99}		&	19			&	25M			&	75			&	2,105		&	15		&	10.67 	\\
{\it as-Skitter}		&	67	&	24385.73		&	*			&	-		&	{\bf 3838.36}	&	1M			&	6M			&	981K		&	737M		&	66		&	27.08 	\\ %1,656,570	737,899,486
{\it roadNet-CA}	&	4	&	*			&	*			&	-		&	{\bf 0.44}		&	1M			&	1M			&	370K		&	4,302		&	4		&	0.08 		\\ %1,487,640
{\it kkt\_power}		&	11	&	*			&	*			&	-		&	{\bf 2.26}		&	1M			&	4M			&	401K		&	2M			&	11		&	1.83 		\\ %1,166,311	 1,978,595
\midrule
{\it rmat\_er\_1}		&	3	&	256.37		&	215.18		&	49.79	&	{\bf 0.38}		&	780			&	1M			&	915			&	8,722		&	3		&	0.12 		\\
{\it rmat\_er\_2}		&	3	&	1016.70		&	865.18		&	-		&	{\bf 0.78}		&	2,019		&	2M			&	2,351		&	23K			&	3		&	0.24 		\\
{\it rmat\_er\_3}		&	3	&	4117.35		&	3456.39		&	-		&	{\bf 1.87}		&	4,349		&	4M			&	4,960		&	50K			&	3		&	0.49 		\\
{\it rmat\_er\_4}		&	3	&	16419.80		&	13894.52		&	-		&	{\bf 4.16}		&	9,032		&	8M			&	10K			&	106K		&	3		&	1.44 		\\
{\it rmat\_er\_5}		&	3	&	*			&	*			&	-		&	{\bf 9.87}		&	18K			&	16M			&	20K			&	212K		&	3		&	2.57 		\\
\midrule
{\it rmat\_sd1\_1}	&	6	&	225.93		&	214.99		&	50.08	&	{\bf 1.39}		&	39K			&	1M			&	23K			&	542K		&	6		&	0.45 		\\
{\it rmat\_sd1\_2}	&	6	&	912.44		&	858.80		&	-		&	{\bf 3.79}		&	90K			&	2M			&	56K			&	1M			&	6		&	0.98 		\\ %1,399,314	
{\it rmat\_sd1\_3}	&	6	&	3676.14		&	3446.02		&	-		&	{\bf 8.17}		&	176K		&	4M			&	106K		&	2M			&	6		&	1.78 		\\ %2,677,437
{\it rmat\_sd1\_4}	&	6	&	14650.40		&	13923.93		&	-		&	{\bf 25.61}		&	369K		&	8M			&	214K		&	5M			&	6		&	4.05 		\\ %5,566,602
{\it rmat\_sd1\_5}	&	6	&	*			&	*			&	-		&	{\bf 46.89}		&	777K		&	16M			&	455K		&	12M			&	6		&	9.39 		\\ %12,168,698
%\midrule
{\it rmat\_sd2\_1}	&	26	&	427.41		&	213.23		&	{\bf 48.17}	&	242.20		&	110K		&	853K		&	88K			&	614M		&	26		&	32.83 	\\ %614,813,037
{\it rmat\_sd2\_2}	&	35	&	4663.62		&	{\bf 851.84}	&	-		&	3936.55		&	232K		&	1M			&	195K		&	1B			&	35		&	95.89 	\\ %1,044,068,886
{\it rmat\_sd2\_3}	&	39	&	13626.23		&	{\bf 3411.14}	&	-		&	10647.84		&	470K		&	3M			&	405K		&	1B			&	37		&	245.51 	\\ %1,343,563,239
{\it rmat\_sd2\_4}	&	43	&	*			&	{\bf 13709.52}	&	-		&	*			&	*			&	*			&	*			&	*			&	42		&	700.05 	\\
{\it rmat\_sd2\_5}	&	N	&	*			&	*			&	-		&	*			&	*			&	*			&	*			&	*			&	51		&    1983.21 	\\
%\vspace*{\rowspace}
\midrule
{\it hamming6-4}	&	4	&	{\bf $<$0.01}	&	{\bf $<$0.01}	&{\bf $<$0.01}	&	{\bf$<$0.01}		&	0			&	704			&	0			&	0			&	4		&	$<$0.01 	\\
{\it johnson8-4-4}	&	14	&	0.19			&	{\bf $<$0.01}	&{\bf $<$0.01}	&	0.23			&	0			&	1,855			&	0			&	0			&	14		&	$<$0.01 	\\
{\it keller4}		&	11	&	22.19		&	0.15			&	{\bf 0.02}	&	23.35		&	0			&	9,435			&	0			&	0			&	11		&	$<$0.01 	\\
{\it c-fat200-5}		&	58	&	0.60			&	0.33			&	{\bf 0.01}	&	0.93			&	0			&	8,473			&	0			&	0			&	58		&	0.04 		\\
{\it brock200\_2}	&	12	&	0.98			&	0.02			&{\bf $<$0.01}	&	1.10			&	0			&	9,876			&	0			&	0			&	10		&	$<$0.01 	\\
\bottomrule\bottomrule
\end{tabular}
%\vspace{-6pt}

\end{table}

